Regular Cost Functions, Part I: Logic and Algebra over Words

The theory of regular cost functions is a quantitative extension to the classical notion of regularity. A cost function associates to each input a non-negative integer value (or infinity), as opposed to languages which only associate to each input the two values "inside" and "outside". This theory is a continuation of the works on distance automata and similar models. These models of automata have been successfully used for solving the star-height problem, the finite power property, the finite substitution problem, the relative inclusion star-height problem and the boundedness problem for monadic-second order logic over words. Our notion of regularity can be -- as in the classical theory of regular languages -- equivalently defined in terms of automata, expressions, algebraic recognisability, and by a variant of the monadic second-order logic. These equivalences are strict extensions of the corresponding classical results. The present paper introduces the cost monadic logic, the quantitative extension to the notion of monadic second-order logic we use, and show that some problems of existence of bounds are decidable for this logic. This is achieved by introducing the corresponding algebraic formalism: stabilisation monoids.

==> computation-trees.tex <==
% !TEX root =  stabilisation_monoids_v4_final.tex



\subsection{Computations, under-computations and over-computations}
\mylabel{subsection:computations}

Our goal is now to provide a formal meaning for the notion of
stabilisation semigroups and stabilisation monoids,
allowing to avoid terms such as ``a lot'' or ``a few''.
More precisely, we develop in this section the notion of computations.
A computation is a tree which is used as a witness that a word
evaluates to a given value.

We fix ourselves for the rest of the section a stabilisation semigroup
$\semigroup=\langle S,\cdot,\sharp,\leq\rangle$.
We develop first the notion for semigroups, and then see how to
use it for monoids in Section~\ref{subsection:monoid-computations}
(we will see that the notions are in close correspondence).

%We start by describing the notion of computation for semigroups.
Let us consider a word $u\in S^+$ (it is a word over $S$, seen as an alphabet).
Our objective is to define a ``value'' for this word. 
In standard semigroups, the ``value'' of $u$ is simply~$\pi(u)$, the product of
the elements appearing in the word. But, what should the ``value'' be for a stabilisation
semigroup?
All the informal semantics we have seen so far were
based on the distinction between ``a few'' and
``a lot''. This means that the value the word has depends on what is
considered as ``a few'', and what is considered as ``a lot''. This is captured
by the fact that the value is parameterised by a positive integer~$n$
which can be understood as a \intro{threshold} separating what is considered
as ``a few'' from what is considered as ``a lot''. For each choice of~$n$,
the word~$u$ is subject to have a different value in the stabilisation
semigroup.

%Consider for instance the stabilisation monoid which counts the number
%of occurrences of the letter~$a$
%(Example~\ref{example:stabilisation-monoid-counta}).
%Imagine now that you want to evaluate the word~$u=a^{10000}$ ($a$ can
%be seen here either as a letter of the alphabet or as an element of the
%stabilisation monoid). This word has value~$a$ for a threshold~$n$
%which is `big' in front of~$10000$, or it can have value~$0$ if~$10000$
%is considered as `big' in front of~$n$. 
%However, those notions have to be treated with care. Indeed, what happens
%around~$n$ is not exactly specified. There is a kind of grey zone around
%$n$. Its origin lies in the intrinsic imprecision of the method, and will appear
%clearly in what follows.

Let us assume a threshold value~$n$ is fixed. We still lack a general mechanism
for associating to each word~$u$ over~$S$ a value in~$S$.
This is the purpose of \intro{computations}.
Computations are proofs (taking the form of a tree) that a
word should evaluate to a given value.
Indeed, in the case of usual semigroups, the fact that a word~$u$ evaluates
to~$\pi(u)$ can be witnessed by a binary tree, the leaves of which, read
from left to right, yield the word~$u$, and such that each inner node is
labelled by the product of the label of its children. Clearly, the root
of such a tree is labelled by~$\pi(u)$, and the tree can be seen as
a proof of correctness for this value.

The notion of $n$-computation that we define now is a variation around
this principle. For more ease in its use, it comes in three variants:
under-computations, over-computations and computations.
\begin{figure}
\begin{center}
%\rogne{0.2cm}{0.3cm}{2cm}{0cm}{
\includegraphics[scale=0.5]{./fig_counta-4-arbre-0.pdf}

%\rogne{0.2cm}{0.3cm}{0cm}{2cm}{
\includegraphics[scale=0.5]{./fig_counta-4-arbre-0-second.pdf}%}
\end{center}
\caption{Two $4$-computations for the word $\mathit{babbbabbbbbaaa}$ in the
monoid of Example~\ref{example:stabilisation-monoid-counta}.}
\mylabel{fig:calculs}
\end{figure}

\begin{definition} An \intro{$n$-under-computation~$T$ for the word~$u=a_1\dots a_l\in S^+$}
is an ordered unranked tree with $l$ leaves, each node~$x$ of which is labelled by
an element~$v(x)\in S$ called the \intro{value of~$x$}, and such that
for all nodes~$x$ of children $y_1,\dots,y_k$ (read from left to right), one
of the following cases holds:
\begin{description}
\item[Leaf] $k=0$, and $v(x)\leq a_m$ where $x$ is the $m$th leave of $T$ (read from left to right),
\item[Binary node] $k=2$, and~$v(x)\leq v(y_1)\cdot v(y_2)$,
\item[Idempotent node] $2\leq k\leq n$ and~$v(x)\leq e$ where $e=v(y_1)=\dots=v(y_k)\in E(M)$,
\item[Stabilisation node] $k>n$ and $v(x)\leq e^\sharp$ where $e=v(y_1)=\dots=v(y_k)\in E(M)$.
\end{description}
An \intro{$n$-over computation} is obtained by replacing everywhere ``$v(x)\leq$''
	by ``$v(x)\geq$''.
An \intro{$n$-computation} is obtained by replacing everywhere ``$v(x)\leq$'' by ``$v(x)=$'', {\it i.e.},
a $n$-computation is a tree which is at the same time
an $n$-under computation and an $n$-over computation.

The \intro{value} of a [under-/over-]computation is the value of its root.

We also use the following notations for easily denoting constructions of [under/over]-computations.
Given a non-leaf $S$-labelled tree $T$, denote by $T^i$ the subtree of $T$
rooted at the $i^\text{th}$ children of the root.
For $a$ in $S$, we note as $a$ the tree restricted
to a single leaf of value $a$. If furthermore $T_1,\dots,T_k$ are also $S$-labelled trees,
then $a[T_1,\dots,T_k]$ denotes the tree of root labelled $a$, of degree $k$,
and such that $T^i=T_i$ for all $i=1\dots k$.
\end{definition}


It should be immediately clear that these notions have
to be manipulated with care, as shown by the following example.
\begin{example} 
Two examples of computations are given in Figure~\ref{fig:calculs}.
Both correspond to the stabilisation semigroup (in fact monoid)
of Example~\ref{example:stabilisation-monoid-counta},
the aim of which is to count the number of occurrences of the letter~$a$ 
in a word. Both correspond to the evaluation of the same word.
Both correspond to the same threshold value~$n$.
However, these two computations do not have the same value.
We will see below how to compare computations and overcome
this problem.
\end{example}

There is another problem. Indeed, it is straightforward to construct an $n$-computation
for some word, simply by constructing a computation which is a binary tree, and
would use no idempotent nodes nor stabilisation nodes.
However, such a computation would of course not be satisfactory since 
every word $u$ would be evaluated in this way as $\pi(u)$.
We do not want that. This would mean that the quantitative aspect contained in the stabilisation has been lost.
We need to determine what is a relevant computation in order to rule out such computations.

Thus we need to answer the following questions:
\begin{enumerate}
\item What are the relevant computations?
\item Can we construct a relevant $n$-computation for all words and all~$n$?
\item How do we relate the different values that $n$-computations may have on
	the same word?
\end{enumerate}

The answer to the first question is that we are only interested in computations
of small height, meaning of height bounded by some function of the semigroup.
With such a restriction, it is not possible to use binary trees as computations.
However, this choice makes the answer to the second question less obvious:
does there always exist a computation?
\begin{theorem}\mylabel{theorem:exists-computation}
For all words~$u\in S^+$ and all non-negative integers~$n$,
there exists an $n$-computation of height at
most\footnote{When measuring the height of a tree, the convention
	is that leaves do not count. With this convention, substituting a tree for a leaf of another tree
	results in a tree of height the sum of the heights of the two trees.} $3|S|$.
\end{theorem}
This result is an extension of the forest factorisation theorem of Simon~\cite{Simon90}
(which corresponds to the case of a semigroup). Its proof,
which is independent from the  rest of this work, is presented in
Section~\ref{subsection:proof-exists-computation}.

\begin{figure}[ht]
\begin{center}
\null\hspace{-5cm}
\includegraphics[scale=1]{./structure-computations.pdf}
\hspace{-5cm}\null
\end{center}
\caption{Structure of computations, under-computations, and over-computations.\mylabel{figure:structure-computations}}
\end{figure}

The third question remains: how to compare the values of different
computations over the same word? An answer to this question  in its full generality makes use
of under- and over-computations.
\begin{theorem}\mylabel{theorem:unicity-computations}
For all non-negative integers~$p$, there exists a polynomial~$\alpha:\nats\rightarrow\nats$
such that for all $n$-under-computations over some word of value~$a$ and
height at most~$p$, and all $\alpha(n)$-over computations of value~$b$
over the same word~$u$,
$$a\leq b\ .$$ 
\end{theorem}
Remark first that since computations are special instances of under- and
over-compu\-tations, Theorem~\ref{theorem:unicity-computations}
holds in particular for comparing the values of compu\-tations.
The proof of Theorem~\ref{theorem:unicity-computations} is the subject of
Section~\ref{subsection:proof-unicity-computations}. 

We have illustrated the above results in Figure~\ref{figure:structure-computations}.
It depicts the relationship between computations in some idealised stabilisation monoid $\semigroup$.
In this drawing, assume some word over some stabilisation semigroup is fixed,
as well as some integer~$p\geq 3|\semigroup|$.
We aim at representing for each~$n$ the possible values of
an $n$-computation, an $n$-under computation or an $n$-over
computation for this word of height at most $p$.
In all the explanations below, all computations are supposed to
not exceed height~$p$.

The horizontal axis represents the $n$-coordinate.
The values in the stabilisation semigroup being ordered,
the vertical axis represents the values in the stabilisation semigroup (for the picture, we
assume the values in the stabilisation semigroup totally ordered).
Thus an $n$-computation (or $n$-under or $n$-over-computation) is placed
at a point of horizontal coordinate $n$ and vertical coordinate the value
of the computation.

We can now interpret the properties of the computations in terms of this figure.
First of all, under-computations as well as over-computations, and as opposed to
computations, enjoy certain forms of monotonicity
as shown by the fact below.
\begin{myfact}\mylabel{fact:under-over-computation-monotonicity}
For~$m\leq n$, all $m$-under-computations are also $n$-under-computations,
and all $n$-over-computations are also $m$-over-computations (using the fact that $e^\sharp\leq e$
for all idempotents $e$).

Any $n$-under-computation of value~$a$ can be turned into an $n$-under-computation
of value $b$ for all $b\leq a$ (by changing the root label from $a$ to $b$).
Similarly any $n$-over-computation of value~$a$ can be turned into an
$n$-over-computation of value $b$ for all $b\geq a$.
\end{myfact}
Fact~\ref{fact:under-over-computation-monotonicity} is illustrated
by Figure~\ref{figure:structure-computations}.
It means that over-computations define a left and upward-closed area, while the under-computations
define a right and downward-closed area. Hence, in particular, the delimiting lines
are non-decreasing.
Furthermore, since computations are at the same-time
over-computations and under-computations, the area of computations lie inside
the intersection of under-compu\-ta\-tions and over-com\-pu\-ta\-tions. 
Since the height~$p$ is chosen to be at least $3|\semigroup|$,
Theorem~\ref{theorem:exists-computation} provides for us even more information.
Namely, for each value of $n$, there exists an $n$-computation.
This means in the picture that the area of computations crosses every column.
However, since computations do not enjoy monotonicity properties, the shape
of the area of computations can be quite complicated.
Finally Theorem~\ref{theorem:unicity-computations} states that the frontier
of under-computations and the frontier of over-computations are not far one
from each other. More precisely, if we choose an element $a$
of the stabilisation semigroup, and we draw an horizontal line at altitude~$a$,
if the frontier of under-computations is above or at $a$ for threshold $n$,
then the frontier of over-computations is also above or at $a$
at threshold $\alpha(n)$. Hence the frontier of over-computations is always below
the one of under-computations, but it essentially grows at the same
speed, with a delay of at most $\alpha$.

\begin{remark}\mylabel{remark:computations-standard}
In the case of standard semigroups or monoids (which can be seen as
stabilisation monoids or semigroups according to Remark~\ref{remark:standard-monoid}),
the notions of computations, under-computations and
over-computations coincide (since the order is trivial),
and the value of the threshold $n$ becomes also
irrelevant. This means that the value of all $n$-[under/over-]computations
over a word~$u$ coincide with $\pi(u)$. (Such computations coincide with
the ``Ramsey factorisations'' of the factorisation forest theorem.)
\end{remark}



Let us finally remark that Theorem~\ref{theorem:unicity-computations}, which is a consequence
of the axioms of stabilisation semigroups, is also sufficient for deducing them.
This is formalised by the following proposition.
\begin{proposition}\mylabel{proposition:unicity-to-axioms}
Let $\semigroup=\langle S,\cdot,\leq,\sharp\rangle$ be a a structure consisting of a finite set $S$,
a binary operation $\cdot$ from $S^2$ to $S$, $\leq$ be a partial order, and $\sharp$
from $S$ to $S$ be a mapping defined over the idempotents of $S$.
Assume furthermore that there exists $\alpha$ such that for all $n$-under-computations for
some word~$u$ of value $a$ of height at most $3$
and all $\alpha(n)$-over-computation over $u$ of
value $b$ of height at most $3$,
$$a\leq b\ .$$

Then $\semigroup$ is a stabilisation semigroup.
\end{proposition}
\begin{proof}
Let us first prove that $\cdot$ is compatible with $\leq$.
Assume $a\leq a'$ and $b\leq b'$, then $(a\cdot b)[a,b]$ is a $0$-under-computation
over $ab$ and $(a'\cdot b')[a',b']$ is an $\alpha(0)$-over-computation over the same
word $ab$. It follows that $a\cdot b\leq a'\cdot b'$.

Let us now prove that $\cdot$ is associative.
Let $a,b,c$ in $n$. Then $((a\cdot b)\cdot c)[(a\cdot b)[a,b],c]$ is a $0$-computation
for the word $abc$, and $(a\cdot(b\cdot c))[a,(b\cdot c)[b,c]]$ is an $\alpha(0)$-computation
for the same word. It follows that $(a\cdot b)\cdot c\leq a\cdot(b\cdot c)$.
The other inequality is symmetric.


Let $e$ be an idempotent. The tree $e^\sharp[\overbrace{e,\dots,e}^{2\alpha(0)+2}]$
is both a $0$ and $\alpha(0)$-computation over the word $e^{2\alpha(0)+1}$.
Furthermore, the tree $(e^\sharp\cdot e^\sharp)[e^\sharp[\overbrace{e,\dots,e}^{\alpha(0)+1}],e^\sharp[\overbrace{e,\dots,e}^{\alpha(0)+1}]]$ is also both a $0$ and an $\alpha(0)$-computation for the same
word. It follows that $e^\sharp\cdot e^\sharp=e^\sharp$, {\it i.e.}, that $\sharp$ maps idempotents to
idempotents.

Let us show that $e^\sharp\leq e$ for all idempotents~$e$.
The tree $e^\sharp[e,e,e]$ is a $2$-computation over the word $eee$,
and $e[e,e,e]$ is a $max(3,\alpha(2))$-computation over the same word.
It follows that $e^\sharp\leq e$.

Let us show that stabilisation is compatible with the order.
Let $e\leq f$ be idempotents.
Then $e^\sharp[\overbrace{e,\dots,e}^{\alpha(0)+1}]$
and $f^\sharp[\overbrace{f,\dots,f}^{\alpha(0)+1}]$ are respectively
a $0$-computation for the word $e^{\alpha(0)+1}$ and 
an $\alpha(0)$-over-computation for the same word. It follows that $e^\sharp\leq f^\sharp$.

Let us prove that stabilisation is idempotent.
Let $e$ be an idempotent. We already know that $(e^\sharp)^\sharp\leq e^\sharp$ (this makes sense since we have
seen that $e^\sharp$ is idempotent). Let
us prove the opposite inequality. 
Consider the $0$-computation $e^\sharp[\overbrace{e,\dots,e}^{(\alpha(0)+1)^2}]$ for the
word $e^{(\alpha(0)+1)^2}$, and the $\alpha(0)$-computation
$(e^\sharp)^\sharp[\overbrace{e^\sharp[\overbrace{e,\dots,e}^{\alpha(0)+1}],
	\dots,e^\sharp[\overbrace{e,\dots,e}^{\alpha(0)+1}]}^{\alpha(0)+1}]$
for the same word. It follows that $e^\sharp\leq (e^\sharp)^\sharp$.

Let us finally prove the consistency of stabilisation.
Assume that both $a\cdot b$ and $b\cdot a$ are idempotents.
Let $t_{ab}$ be $(a\cdot b)[a,b]$ (and similarly for $t_{ba}$), {\it i.e.}, computations for $ab$ and $ba$
respectively.
Define now:
\begin{align*}
	t_{(a\cdot b)^\sharp}&=
		(a\cdot b)^\sharp[\overbrace{t_{ab},\dots,t_{ab}}^{\alpha(0)+2~\text{times}}]\ ,\\
\text{and} \qquad
t_{a\cdot (b\cdot a)^\sharp\cdot b}&=(a\cdot (b\cdot a)^\sharp\cdot b)[
		a,((b\cdot a)^\sharp\cdot b)[
			(b\cdot a)^\sharp[\overbrace{t_{ba},\dots,t_{ba}}^{\alpha(0)+1~\text{times}}]
			,b]]\ .\\
\end{align*}
Then both $t_{(a\cdot b)^\sharp}$ and $t_{a\cdot (b\cdot a)^\sharp\cdot b}$
are at the same time $0$ and $\alpha(0)$-computations over the same word $(ab)^{\alpha(0)+2}$
of height at most~$3$.
Since their respective values are $(a\cdot b)^\sharp$ and $a\cdot (b\cdot a)^\sharp\cdot b$,
it follows by our assumption that $(a\cdot b)^\sharp=a\cdot (b\cdot a)^\sharp\cdot b$.
\end{proof}
This result is particularly useful. Indeed, when constructing a new stabilisation semigroup,
we usually aim at proving that it ``recognises'' some function (to be defined in the next chapter). 
It involves proving the hypothesis of Proposition~\ref{proposition:unicity-to-axioms}. Thanks to
Proposition~\ref{proposition:unicity-to-axioms}, the syntactic correctness is then for free.
This situation occurs in particular in Section~\ref{subsection:closure-inf-projection}
and \ref{subsection:closure-sup-projection} when the closure of recognisable
cost-functions under inf-projection and sup-projection is established.



\subsection{Specificities of stabilisation monoids}
\mylabel{subsection:monoid-computations}

We have presented so far the notion of computations in the case of stabilisation semigroups.
We are in fact interested in the study of stabilisation monoids.
Monoids differ from semigroups by the presence of a unit element~$1$.
This element is used for modelling the empty word.
We present in this section the natural variant of the notions of computations
for the case of stabilisation monoids. As is often the case, results from stabilisation
semigroups transfer naturally to stabilisation monoids.
The definition is highly related to the one for stabilisation semigroups,
and we see through this section that it is easy to go from the notion
for stabilisation monoid to the one of stabilisation semigroup case, and backward.
The result is that we use the same name ``computation'' for the two notions elsewhere
in the paper.
\begin{definition}
Let $\monoid$ be a stabilisation monoid.
Given a word $u\in M^*$, a \intro{stabilisation monoid $n$-[under/over]-computation} (\intro{sm}-[under/over]-computation
for short) for $u$
is an $n$-[under/over]-computation for some $v\in M^+$,
such that it is possible to obtain $u$ from $v$ by deleting some occurrences of the
letter $1$. All have value $1$.
\end{definition}
Thus, the definition deals with the implicit presence of arbitrary many copies of the
empty word (the unit) interleaved with a given word.
This definition allows us to work in a transparent way with the empty word (this saves us
case distinctions in proofs). In particular the empty word has an 
sm-$n$-computation which is simply $1$, of value $1$. 
There are many others, like $1[1,1,1,1[1,1]]$ for instance.

Since each $n$-computation is also an sm-n-computation over the same word,
it is clear that Theorem \ref{theorem:exists-computation} can be extended to this situation (just the
obvious case of the empty word needs to be treated separately):
\begin{myfact}\mylabel{fact:exists-SM-computation}
There exists an sm-$n$-computation for all words in $M^*$
of size at most $3|M|$.
 \end{myfact}

The following lemma shows that sm-[under/over]-computations are not more expressive than
[under/over]-computations. It is also elementary to prove.
\begin{lemma}\mylabel{lemma:remove-epsilon-computation}
Given an sm-$n$-computation
({\it resp.}, sm-$n$-under-computation, sm-$n$-over-com\-putation)
of value $a$ for the empty word,  then $a=1$ ({\it resp.} $a\leq 1$, $a\geq 1$).

For all non-empty words $u$ and all sm-$n$-computations $T$
({\it resp.}, sm-$n$-under-computa\-tions, sm-$n$-over-computations)
for $u$ of value $a$, there exists an  $n$-computation
({\it resp.}, $n$-under-computations, $n$-over-computations) for $u$ of value $a$. Furthermore, its height is at most the height of $T$.
\end{lemma}
\begin{proof}
It is simple to eliminate each occurrence of an extra $1$ by local modifications of the structure of the sm-computation:
replace subtrees of the form $1[1,\dots,1]$ by $1$, subtrees of the form $a[T,1]$ by $T$, and subtrees of the form  $a[1,T]$ by $T$,
up to elimination of all occurrences of $1$.
For the empty word, this results in the first part of the lemma. For non-empty words, the resulting simplified
sm-computation is a computation. The argument works identically for the under/over variants.
\end{proof}
A corollary is that Theorem~\ref{theorem:unicity-computations} extends to sm-computations.
\begin{corollary}
For all non-negative integers~$p$, there exists a polynomial~$\alpha:\nats\rightarrow\nats$
such that for all sm-$n$-under-computations over some word $u\in M^*$ of value~$a$ and
height at most~$p$, and all sm-$\alpha(n)$-over computations of value~$b$
over the same word~$u$,
$$a\leq b\ .$$ 
\end{corollary}
\begin{proof}
Indeed, the sm-under-computations and sm-over-computations can be turned into
under-computations and over-computations of the same respective values by
Lemma~\ref{lemma:remove-epsilon-computation}.
The inequality holds for these under and over-computations by  Theorem~\ref{theorem:unicity-computations}.
\end{proof}

There is a last lemma which is related and will prove useful.
\begin{lemma}\mylabel{lemma:SM-extension}
Let $u$ be a word in $M^*$ and $v$ be obtained from $u$ by eliminating some of its $1$ letters,
then all $n$-[under/over]-computations for $v$ can be turned into an $n$-[under/over]-computation for $u$
of same value. Furthermore, the height increase is at most $3$.
\end{lemma}
\begin{proof}
Let $v=a_1\dots a_n$, then $u=u_1\dots u_n$ for $u_i\in 1^*a_i1^*$.
Let $T$ be the $n$-[under/over]-computation for $v$ of value $a$.
It is easy to construct an $n$-[under/over]-computation $T_i$ for $u_i$ of height at most $3$
of value $a_i$. It is then sufficient to plug in $T$ each $T_i$ for the $i$th leave of $T$.
\end{proof}

The consequence of these results is that we can work with sm-[under/over]-computations
as with [under-over]-computations.
For this reason we shall not distinguish further between the two notions unless necessary.






\subsection{Existence of computations: the proof of Theorem~\ref{theorem:exists-computation}}
\mylabel{subsection:proof-exists-computation}

In this section, we establish Theorem~\ref{theorem:exists-computation} which states
that for all words~$u$ over a stabilisation semigroup~$\semigroup$ and all non-negative integers~$n$,
there exists an $n$-computation for~$u$ of height at most~$3|S|$.
Remark that the convention in this context is to measure the height of a tree without counting the leaves.
This result is a form of extension of the factorisation forest theorem
due to Simon \cite{Simon90}:
\begin{theorem}[Simon \cite{Simon90,Simon92}]\mylabel{theorem:factorisation-forest}
Define a \intro{Ramsey factorisation} to be an $n$-computation in the pathological case $n=\infty$
({\it i.e.}, there are no stabilisation nodes, and idempotent nodes are allowed to have arbitrary degree).

\noindent
For all non-empty words~$u$ over a finite semigroup~$\semigroup$, there exists a Ramsey factorisation
for~$u$ of height\footnote{The exact bound of $3|S|-1$ is due to Kufleitner \cite{Kufleitner08}.
It is likely that the same bound could be achieved for Theorem~\ref{theorem:exists-computation}.
We prefer here a simpler proof with a bound of $3|S|$.} at most~$3|\semigroup|-1$.
\end{theorem}
Some proofs of the factorisation forest theorem can be found in \cite{Kufleitner08,TCS10:colcombet-fct,LATA11:colcombet}.
Our proof could follow similar lines as the above one. Instead of that,
we try to reuse as much lemmas as possible from the above constructions.

For proving Theorem~\ref{theorem:exists-computation}, we will need one of Green's relations,
namely the $\gJ$-relation (while there are five relations in general).
Let us fix ourselves a semigroup~$\semigroup$.
We denote by $\semigroup^1$ the semigroup extended (if necessary)
with a neutral element $1$ (this transforms $\semigroup$ into a monoid).
Given two elements $a,b\in S$, $a \leq_\gJ b$ if~$a=x\cdot b\cdot y$ for some~$x,y\in S^1$.
If $a\leq_\gJ b$ and~$b\leq_\gJ b$, then~$a \gJ b$.
We write~$a<_\gJ b$ to denote~$a\leq_\gJ b$ and~$b\not\leq_\gJ a$.
The interested reader can see, {\it e.g.}, \cite{LATA11:colcombet}
for an introduction to the relations of Green (with a proof of the factorisation forest theorem),
or monographs such as~\cite{Lallement79}, \cite{Grillet95} or \cite{Pin86} for deep presentations
of this theory.
Finally, let us call a \intro{regular element}
in a semigroup an element~$a$ such that~$a\cdot x\cdot a=a$ for some~$x\in S^1$.

The next lemma gathers some classical results concerning finite semigroups.
\begin{lemma}\mylabel{lemma:J-regular}
Given a $\gJ$-class $J$ in a finite semigroup, the following facts are equivalent:
\begin{itemize}
\item $J$ contains an idempotent,
\item $J$ contains a regular element,
\item there exist $a,b\in J$ such that $a\cdot b\in J$,
\item all elements in $J$ are regular,
\item all elements in $J$ can be written as $e\cdot c$ for some idempotent $e\in J$,
\item all elements in $J$ can be written as $c\cdot e$ for some idempotent $e\in J$.
\end{itemize}
Such~$\gJ$-classes are called \intro{regular}. 
\end{lemma}
We will use the following technical lemma.
\begin{lemma}\mylabel{lemma:J-idempotent}
If $f=e\cdot x\cdot e$ for $e\gJ f$ two idempotents, then $e=f$.
\end{lemma}
\begin{proof}
We use some standard results concerning finite semigroups.
The interested reader can find the necessary material for instance in \cite{Pin86}.
Let us just recall that the relations $\leq_\gL$, $\leq_\gR$ and $\gL$ and $\gR$
are the one-sided variants of $\leq_\gJ$ and $\gJ$ ($\gL$ stands for ``left'' and $\gR$ for ``right'').
Namely, $a\leq_\gL b$ ({\it resp.} $a\leq_\gR b$) holds if $a=x\cdot b$ for some $x\in S^1$ ({\it resp.} $a=b\cdot x$),
and $\gL=\leq_\gL\cap\geq_\gL$ ({\it resp.} $\gR=\leq_\gR\cap\geq_\gR$).
Finally, $\gH=\gL\cap\gR$.

The proof is very short. By definition $f\leq_\gL e$ since $e\cdot x\cdot e=f$.
Since by assumption $f\gJ e$, we obtain $f\gL e$
(a classical result in \emph{finite} semigroups).
In a symmetric way $f\gR e$. Thus $f\gH e$. Since an $\gH$-class contains at most
one idempotent, $f=e$ (it is classical than any $\gH$-class, when containing an idempotent, has a group structure; since
groups contain exactly one idempotent element, this is the only one).
\end{proof}
The next lemma shows that the stabilisation operation behaves in a very uniform way
inside $\gJ$-classes (similar arguments can be found in the works of Leung, Simon and Kirsten).
\begin{lemma}\mylabel{lemma:stabilisation-preserve-J}
If $e\gJ f$ are idempotents, then $e^\sharp \gJ f^\sharp$. Furthermore, if $e=x\cdot f\cdot y$
for some $x,y$, then $e^\sharp=x\cdot f^\sharp\cdot y$.
\end{lemma}
\begin{proof}
For the second part,
assume $e=x\cdot f\cdot y$ and $e\gJ f$. Let $f'=(f\cdot y\cdot e\cdot x\cdot f)$.
We easily check $f'\cdot f'=f'$.
Furthermore $f\gJ e=(x\cdot f\cdot y)\cdot e\cdot  (x\cdot f\cdot y)\leq_\gJ f'\leq_\gJ f$. Hence $f\gJ f'$.
It follows by Lemma~\ref{lemma:J-idempotent} that $f'=f$.
We now compute $e^\sharp = (x\cdot f\cdot f\cdot y)^\sharp=x\cdot f\cdot(f\cdot x\cdot y\cdot f)^\sharp\cdot f\cdot y=x\cdot f\cdot f^\sharp\cdot f\cdot y=x\cdot f^\sharp\cdot y$ (using consistency and $f=f'$).

This proves that $e\gJ f$ implies $e^\sharp\leq_\gJ f^\sharp$. Using symmetry, we obtain $e^\sharp\gJ f^\sharp$.
\end{proof}
Hence, if $J$ is a regular $\gJ$-class, there exists a unique $\gJ$-class $J^\sharp$
which contains $e^\sharp$ for one/all idempotents $e\in J$. If $J=J^\sharp$,
then $J$ is called \intro{stable}, otherwise, it is called \intro{unstable}.
The following lemma shows that stabilisation is trivial over stable $\gJ$-classes.
\begin{lemma}\mylabel{lemma:stable}
If $J$ is a stable $\gJ$-class, then $e^\sharp=e$ for all idempotents $e\in J$.
\end{lemma}
\begin{proof}
Indeed, we have $e^\sharp=e\cdot e^\sharp\cdot e$ and thus by Lemma~\ref{lemma:J-idempotent}, $e^\sharp=e$. 
\end{proof}
The situation is different for unstable $\gJ$-classes.
In this case, the stabilisation always goes down in the $\gJ$-order.
\begin{lemma}\mylabel{lemma:unstable}
If $J$ is an unstable $\gJ$-class, then $e^\sharp<_\gJ e$ for all idempotents $e\in J$.
\end{lemma}
\begin{proof}
Since $e^\sharp=e\cdot e^\sharp$, it is always the
case that $e^\sharp\leq_\gJ e$. Assuming $J$ is unstable means that $e\gJ e^\sharp$
does not hold, which in turn implies $e^\sharp<_\gJ e$.
\end{proof}



We say that a word~$u=a_1\dots a_n$ in $S^+$
is \intro{$J$-smooth}, for $J$ a $\gJ$-class,
if $u\in J^+$, and $\pi(u)\in J$.
It is equivalent to say that  $\pi(a_ia_{i+1}\cdots a_j)\in J$ for all $1\leq i<j\leq n$.
Indeed for all $1\leq i<j\leq n$, $a_i\gJ \pi(a_1\dots a_n)\leq_\gJ \pi(a_ia_{i+1}\cdots a_j)\leq_\gJ a_i\in J$.
Remark that, according to Lemma~\ref{lemma:J-regular}, if $J$ is irregular,
$J$-smooth words have length at most $1$. 
We will use the following lemma from \cite{LATA11:colcombet} as a black-box.
This is an instance of the factorisation forest theorem, but restricted to
a single $\gJ$-class.
\begin{lemma}[{Lemma~14 in \cite{LATA11:colcombet}}]\mylabel{lemma:factorisation-J}
Given a finite semigroup $\semigroup$, one of its $\gJ$-classes $J$, and a $J$-smooth word~$u$,
there exists a Ramsey factorisation for $u$ of height at most $3|J|-1$. 
\end{lemma}

Remark that Ramsey factorisations and $n$-computations do only differ on what is allowed for a node
of large degree, {\it i.e.}, above $n$. That is why our construction makes use of Lemma~\ref{lemma:factorisation-J}
to produce Ramsey factorisations, and then based on the presence of nodes of large degree, constructs
a computation by gluing pieces of Ramsey factorisations together.
\begin{lemma}\mylabel{lemma:computation-base}
Let $J$ be a $\gJ$-class, $u$ be a $J$-smooth word, and $n$ be some non-negative integer.
Then one of the two following items holds:
\begin{enumerate}
\item there exists an $n$-computation for $u$ of value $\pi(u)$ and height at most $3|J|-1$, or;
\item there exists an $n$-computation for some non-empty prefix $w$ of $u$ of value\footnote{A closer
		inspection would reveal that $a\in J^\sharp$. This extra information is useless for our purpose.}
	$a<_\gJ J$ and height at most $3|J|$.
\end{enumerate}
\end{lemma}
\begin{proof}
Remark that if $J$ is irregular, then $u$ has length $1$ by Lemma~\ref{lemma:J-regular},
and the result is straightforward.
Remark also that if $J$ is stable, and since the stabilisation is trivial in stable $\gJ$-classes
(Lemma~\ref{lemma:stable}),
every Ramsey factorisations for $u$ of height at most
$3|J|-1$ (which exist by Lemma~\ref{lemma:factorisation-J}) is in fact $n$-computations for $u$.

The case of $J$ unstable remains.
Let us say that a node in a factorisation is \intro{big} if its degree is more than $n$.
Our goal is to ``correct'' the value of big nodes.
If there is a Ramsey factorisation for $u$ which has no big node, then it can be seen
as an $n$-computation, and once more the first conclusion of the lemma holds.

Otherwise, consider the least non-empty prefix $u'$ of $u$ for which there is a  Ramsey factorisation of height 
at most $3|J|-1$ which contains a big node. Let $F$ be such a factorisation and $x$ be a big node in $F$
which is maximal for the descendant relation (there are no other big nodes below).
Let $F'$ be the subtree of $F$ rooted in $x$.
This decomposes $u'$ into $vv'v''$ where $v'$ is the factor of $u'$ for which $F'$ is a Ramsey factorisation.
For this $v'$, it is easy to transform $F'$ into an $n$-computation $T'$ for $v'$: just replace the label $e$ of the
root of $F'$ by $e^\sharp$. Indeed, since there are no other big nodes in $F'$ than the root, the root is the only place
which prevents $F'$ from being an $n$-computation. Remark that from Lemma~\ref{lemma:unstable},
the value of $F'$ is $<_\gJ J$.

If $v$ is empty, then $v'$ is a prefix of $u$, and $F'$ an $n$-computation for it. The second conclusion of the lemma holds.

Otherwise, by the minimality assumption and Lemma~\ref{lemma:factorisation-J},
there exists a Ramsey factorisation $T$ for $v$ of height at most $3|J|-1$ which contains no
big node. Both $T$ and $T'$ being $n$-computations of height at most $3|J|-1$,
it is easy to combine them into an $n$-computation of height at most $3|J|$ for $vv'$.
This is an $n$-computation for $vv'$, which inherits from $F'$ the property that its value
is $<_\gJ J$. It proves that the second conclusion of the lemma holds.
\end{proof}

We are now ready to establish Theorem~\ref{theorem:exists-computation}.
 \begin{proof}
 The proof is by induction on the size of a left-right-ideal $Z\subseteq S$, {\it i.e.}, 
$S^1\cdot Z\cdot S^1\subseteq Z$ (remark that a left-right-ideal is a union of $\gJ$-classes).
We establish by induction on the size of $Z$ the following induction hypothesis:
\begin{center}
\emph{IH:} for all words $u\in Z^++Z^*S$ there exists an $n$-computation
of height at most $3|Z|$ for $u$.
 \end{center}
 Of course, for $Z=S$, this proves  Theorem~\ref{theorem:exists-computation}.
 
The base case is when $Z$ is empty, then $u$ has length $1$, and a single node tree
establish the first conclusion of the induction hypothesis 
(recall that the convention is that the leaves do not count in the height,
and as a consequence a single node tree has height $0$).

Otherwise, assume $Z$ non-empty. There exists a maximal $\gJ$-class $J$
(maximal for $\leq_\gJ$) included in $Z$.
From the maximality assumption, we can check that $Z'=Z\setminus J$ is again a left-right-ideal.
Remark also that since $Z$ is a left-right-ideal, it is downward closed for $\leq_\gJ$.
This means in particular that every element $a$ such that $a<_\gJ J$ belongs to $Z'$.


\emph{Claim:} We claim ($\star$) that for all words $u\in Z^++Z^*S$,
\begin{enumerate}
\item either there exists an $n$-computation of height $3|J|$ for $u$, or;
\item there exists an $n$-computation of height at most $3|J|$ for some non-empty prefix
of $u$ of value in $Z'$.
\end{enumerate}

Let $w$ be the longest $J$-smooth prefix of $u$. If there exists no such non-empty prefix, this
means that the first letter $a$  of $u$ does not belong to $J$.
Two subcases can happen.
If $u$ has length $1$, this means that $u=a$, and thus $a$ is an $n$-computation witnessing
the first conclusion of ($\star$). Otherwise $u$ has length at least $2$, and thus $a$ belongs to $Z$.
Since furthermore it does not belong to $J$, it belongs to $Z'$. In this case, $a$ is an $n$-computation
witnessing the second conclusion of ($\star$).

Otherwise, according to Lemma~\ref{lemma:computation-base} applied to $w$, two situations can occur.
The first case is when there is an $n$-computation $T$ for $w$ of value $\pi(w)$ and height
at most $3|J|-1$.
There are several sub-cases.  If $u=w$, of course, the $n$-computation $T$ is a witness
that the first conclusion of ($\star$) holds.
Otherwise, there is a letter $a$ such that $wa$ is a prefix of $u$. 
If $wa=u$, then $\pi(wa)[T,a]$ is an $n$-computation for $wa$ of height at most
$3|J|$, witnessing that the first conclusion of ($\star$) holds.
Otherwise, $a$ has to belong to $Z$ (because all letters of $u$
have to belong to $Z$ except possibly the last one).
But, by maximality of $w$ as a $J$-smooth prefix,
either $a\in Z'$, or $\pi(wa)\in Z'$. Since $Z'$ is a left-right-ideal, $a\in Z'$
implies $\pi(wa)\in Z'$. Then,  $\pi(wa)[T,a]$ is an $n$-computation
for $wa$ of height at most $3|J|$ and value $\pi(wa)\in Z'$. This time,
the second conclusion of ($\star$) holds.

The second case according to Lemma~\ref{lemma:computation-base}
is when there exists a prefix $v$ of $w$
for which there is an $n$-computation of height at most $3|J|$ of value $<_\gJ J$.
In this case, $v$ is also a prefix of $u$, and the value of this computation is in $Z'$.
Once more the second conclusion of ($\star$) holds.
This concludes the proof of Claim~($\star$).
\smallskip

As long as the second conclusion of the claim ($\star$)
applied on the word $u$ holds, this decomposes $u$ into $v_1u'$,
and we can proceed with $u'$.
In the end, we obtain that all words $u\in Z^++Z^*S$ can
be decomposed into $u_1\dots u_k$ such that
there exist $n$-computations $T_1,\dots,T_k$ of height at most $3|J|$
for $u_1,\dots,u_k$ respectively, and such that the values of $T_1,\dots,T_{k-1}$
all belong to $Z'$ (but not necessarily the value of $T_k$).
Let $a_1,\dots,a_k$ be the values of $T_1,\dots,T_k$ respectively.
The word $a_1\dots a_k$ belongs to $Z'^++Z'^*S$.
Let us apply the induction hypothesis to the word $a_1\dots a_k$. We obtain
an $n$-computation $T$ for $a_1\dots a_k$ of height at most $3|Z'|$.
By simply substituting $T_1,\dots,T_k$ to the leaves of $T$, we obtain an
$n$-computation for $u$ of height at most $3|J|+3|Z'|=3|Z|$. (Remark once more
here that the convention is to not count the leaves in the height. Hence the height after
a substitution is bounded by the sum of the heights.)
\end{proof}























\subsection{Comparing computations: the proof of Theorem~\ref{theorem:unicity-computations}}
\mylabel{subsection:proof-unicity-computations}

We now establish the second key theorem for computations, namely
Theorem~\ref{theorem:unicity-computations} which states that the result of computations
is, in some sense, unique. The proof works by a case analysis on the possible
ways the over-computations and under-computations may overlap. 
We perform this proof for stabilisation monoids, thus using sm-computations.
More precisely, all statements take as input computations, and output
sm-computations, which can be then normalised into non-sm computations.
The result for stabilisation semigroup can be derived from it.
We fix ourselves from now on a stabilisation monoid $\monoid$.



\begin{lemma}\mylabel{lemma:over-computation-above-pi}
For all $n$-over-computations of value~$a$ over a word~$u\in M^*$ of length at most~$n$, $\pi(u)\leq a$.
\end{lemma}
\begin{proof}
By induction on the height of the over-computation, using the fact that an $n$-over-computation for a word
of length at most $n$ cannot contain a stabilisation node.
\end{proof}

\begin{lemma}\mylabel{lemma:over-computation-above-sharp}
For all $n$-over-computations of value~$b$
over a word~$b_1 \dots b_k$ ($k\geq 1$) such that~$e\leq b_i$ for all~$i$,
and $e$ is an idempotent, then~$e^\sharp\leq b$.
\end{lemma}
\begin{proof}
By induction on the height of the over-computation.
\end{proof}

A sequence of words $u_1,\dots,u_k$ is called a \intro{decomposition} of~$u$ if~$u=u_1\dots u_k$.
We say that a non-leaf [under/over]-computation~$T$ for a word~$u$ \intro{decomposes} $u$ into~$u_1$,\dots,$u_k$
if the subtree rooted at the $i$th child of the root is an [under/over]-computation for $u_i$, for all $i=1\dots k$.
Our proof will mainly make use of over-computations.
For this reason, we introduce the following terminology.

We say that a word $u\in M^*$ $n$-\intro{evaluates} to $a\in M$ if there exists an $n$-over-computation for $u$
of value $a$. We will also say that $u_1,\dots,u_k$ $n$-evaluate to $b_1,\dots,b_k$
if $u_i$ $n$-evaluates to $b_i$ for all $i=1\dots k$.

This notion is subject to elementary reasoning such as (a) $u$ $n$-evaluates to $\pi(u)$ or (b) if $u_1,\dots,u_k$
$n$-evaluate to $b_1,\dots,b_k$ and $b_1\dots b_k$ $n$-evaluates to $b$, then $u_1\dots u_k$
$n$-evaluates to $b$.

The core of the proof is contained in the following property:

\begin{lemma}\mylabel{lemma:over-computation-decomposition}
There exists a polynomial~$\alpha$ such that for all $u_1,\dots,u_k\in M^*$,
if $u_1\dots u_k$ $\alpha(n)$-evaluates to $b$ then 
$u_1,\dots,u_k$ $n$-evaluate $b_1,\dots,b_k$, and $b_1\dots b_k$ $n$-evaluates to $b$,
for some $b_1,\dots,b_k\in M$.

\ign{
for all $\alpha(n)$-over-computations~$T$ over a word~$u$ of value~$b$,
and all decompositions of $u$ into~$u_1,\dots,u_k$, then:
\begin{enumerate}
\item there exist $n$-over-computations~$B_1$ \dots $B_k$ for $u_1$,\dots,$u_k$ respectively,
	of value $b_1$,\dots,$b_k$ respectively, and,
\item there exists an $n$-over-computation~$B$ over~$b_1\dots b_k$ of value~$b$.
\end{enumerate}}
\end{lemma}
From this result, we can deduce Theorem~\ref{theorem:unicity-computations} as follows.
\begin{proof}[Proof of Theorem~\ref{theorem:unicity-computations}]
Let~$\alpha$ be as in Lemma~\ref{lemma:over-computation-decomposition}.
Let~$\alpha_p$ be the $p$th composition of $\alpha$ with itself. 
Let~$U$ be an $n$-under-computation of height at most $p$ for some word $u$ of value $a$,
and $T$ be an $\alpha_p(n)$-over-computation for $u$ of value $b$. We want to establish that $a\leq b$.
The proof is by induction on~$p$.

If~$p=0$, this means that $u$ has length $1$, then $T$ and $U$ are also restricted to a single leaf, and the
result obviously holds. Otherwise, $U$ decomposes $u$ into $u_1,\dots,u_k$.
Let $a_1$,\dots,$a_k$ be the values of the children of the root of $i$, read from left to right.
By applying Lemma~\ref{lemma:over-computation-decomposition}
on $T$ and the decomposition $u_1,\dots,u_k$. We construct the
$\alpha_{p-1}(n)$-over-computations $B_1,\dots,B_k$ for $u_1,\dots,u_k$ respectively,
and of respective values $b_1,\dots,b_k$,
as well as an $\alpha_{p-1}(n)$-over-computation $B$ of value $b$ for $b_1,\dots,b_k$.

For all $i=1\dots k$, we can apply the induction hypothesis on
$U^i$ (let us recall that $U^i$ is the sub-under-computation rooted at the $i$th child of the root of $U$)
and $B_i$, and obtain that $a_i\leq b_i$. Depending on $k$, three cases
have to be separated.
If $k=2$ (binary node), then $a\leq a_1\cdot a_2\leq b_1\cdot b_2\leq b$.
If $3\leq k\leq n$ (idempotent node), we have $a\leq a_1=\cdots=a_k=e$ which is an idempotent.
We have $e=a_i\leq b_i$ for all $i=1\dots k$. Hence by Lemma~\ref{lemma:over-computation-above-pi},
$e\leq b$, which means $a\leq b$.
If $k>n$  (stabilisation node), we have once more $a_1=\cdots=a_k=e$ which is an idempotent, and 
such that $a\leq e^\sharp$.
This time, by Lemma~\ref{lemma:over-computation-above-sharp}, we have $e^\sharp\leq b$. We obtain
once more $a\leq b$.
\end{proof}

The remainder of this section is dedicated to the proof of Lemma~\ref{lemma:over-computation-decomposition}.


\ign{
We first establish this result for $k$ fixed.

\begin{lemma}\mylabel{lemma:over-computation-bounded-decomposition}
For all positive integers $k$, there exists a polynomial~$\alpha$ such that
for all words $u$ which $\alpha(n)$-evaluate to $b$,
and all decompositions of $u$ into $u_1\dots u_k$,
then $u_1,\dots,u_k$ $n$-evaluate to $b_1,\dots,b_k$
such that $\pi(b_1\ldots b_k)\leq b$.
\end{lemma}
\begin{proof}
Let us treat first the case $k=2$.
Let~$\alpha(n)=2n+1$ and let $T$ be an $\alpha(n)$-over-computation of value $b$ over a word~$u=u_1u_2$.
The proof is by induction on the height of $T$.
Remark first that if $u_1$ or $u_2$ are empty, the result is straightforward.
The case of a leaf is also treated since this means that either $u_1$ or $u_2$ is empty.

Otherwise the over-computation $T$ decomposes $u$ as $v_1,\dots,v_l$.
Let $a_1,\dots,a_l$ be the values of the children of the root.
There exist some $s$ in $1\dots l$ and words $w_1,w_2$ such that:
\begin{align*}
u_1 &= v_1\ldots v_{s-1}w_1\ ,&v_s &= w_1w_2,\ &\text{and}~u_2&=w_2v_{s+1}\dots v_{l}\ .
\end{align*}
We apply the induction hypothesis on $v_s$ decomposed into $w_1,w_2$.
From the induction hypothesis, we get that $w_1,w_2$ $n$-evaluate to $c_1,c_2$
 such that $c_1\cdot c_2\leq a_s$.

If $l=2$ (binary node). Then either $s=1$ or $s=2$. The two cases being symmetric,
let us treat the case $s=1$. In this case, $u_1=w_1,u_2=w_2v_2$
$n$-evaluate to $c_1,c_2\cdot a_2$,
and furthermore $\pi(c_1(c_2\cdot a_2))=(c_1\cdot c_2)\cdot a_2\leq \pi(a_1a_2)$.

If $3\leq l\leq 2n+1$ (case of an idempotent node), then $a_1=\dots=a_l=e$ idempotent,
and $e\leq b$. 
In this case $a_1\dots a_{s-1}$ $n$-evaluates to $e$ (or $1$ if $s=1$).
We get from this that $v_1\dots v_{s-1}$ $n$-evaluates to $e$ (or $1$ if $s=1$) (since each $v_i$ $n$-evaluates
to $a_i$). Hence $u_1=v_1\dots v_{s-1}w_1$ $n$-evaluates to $b_1=e\cdot c_1$ (or $c_1$ if $s=1$).
In the same way $u_2=w_2v_{s+1}\dots v_l$ $n$-evaluates to $b_2=c_2\cdot e$ (or $c_2$ if $s=l$).
Since furthermore $c_1\cdot c_2\leq e$, we obtain $b_1\cdot b_2\leq e\leq b$.

If $l > 2n+2$ (case of a stabilisation node), then $a_1=\dots=a_l=e$ is an idempotent,
and $e^\sharp\leq b$. 
Two situations can occur depending on whether $s$
is on the left or the right half of $u$. Let us treat the case $s>n+1$.
In this case,  $v_1\dots v_{s-1}$ $n$-evaluates to $e^\sharp$,
and thus $u_1=v_1\dots v_{s-1}w_1$ $n$-evaluates to $b_1=e^\sharp\cdot c_1$.
As in the idempotent case $u_2$ $n$-evaluates to $b_2=c_2\cdot e$ (or possibly $c_2$).
Since $c_2\cdot c_2\leq e$, we obtain $b_1\cdot b_2=e^\sharp \cdot c_1 \cdot c_2 \cdot e\leq e^\sharp\le b$.

The case for $k>2$ is easily obtained by induction on $k$ from the above.
Denote by $\alpha^p$ the $p$th composition of $\alpha$ with itself.
Assume $u_1\dots u_k$ $\alpha^p(n)$-evaluates to $b$,
then $u_1\dots u_{k-1},u_k$  $\alpha^{p-1}(n)$ evaluate to $c,b_k$ such that $c\cdot b_k\leq b$
(using the case $k=2$).
Applying the induction hypothesis, we know that $u_1,\dots,u_{k-1}$
$n$-evaluate to $b_1,\dots,b_{k-1}$ such that $\pi(b_1\dots b_{k-1})\leq c$.
It follows that $u_1,\dots,u_{k}$
$n$-evaluate to $b_1,\dots,b_{k}$ with $\pi(b_1\dots b_{k})\leq c\cdot b_k\leq b$.
\end{proof}}


\begin{lemma}\mylabel{lemma:ordered-consistency}
There exists a positive integer $K$ such that for all idempotents $e,f$,
whenever $f\leq a_i\cdot b_i$ for all $i=1\dots k$, $k\geq K$,
and $b_i\cdot a_{i+1}\leq e$ for $i=1\dots k-1$, then $f^\sharp\leq a_1\cdot e^\sharp\cdot b_k$.
\end{lemma}
\begin{proof}
To each ordered pair $i<j$, let us associates the color $c_{i,j}=(a_i,\pi(b_ia_{i+1}\dots b_{j-1}))$.
We now apply the theorem of Ramsey to this coloring, for $K$ sufficiently large,
and get that there exist $1<i<s<j<k$ such that $c_{i,s}=c_{s,j}=_{c_{i,j}}=(a,b)$.
This implies in particular that $b\cdot a\cdot b=b$, and thus $a\cdot b$ and $b\cdot a$
are idempotents. Furthermore, $f\leq a\cdot b$ and $b\cdot a\leq e$.
It follows from consistency that
$f^\sharp\leq (a\cdot b)^\sharp\leq a\cdot (b\cdot a)^\sharp\cdot b\leq a\cdot e^\sharp\cdot b= a_i\cdot e^\sharp\cdot \pi(b_s\dots b_{j-1})$.
We now have, using the assumptions that $f\leq a_h\cdot b_h$ and $b_h\cdot a_{h+1}\leq e$,
\begin{align*}
f^\sharp	&=f\cdot f^\sharp\cdot f\leq \pi(a_1\dots a_i)\cdot e^\sharp\cdot \pi(b_s\dots b_k)
		\leq a_1\cdot e\cdot e^\sharp\cdot e\cdot b_k=a_1\cdot e^\sharp\cdot  b_k\ .
\end{align*}
\end{proof}

The following lemma will be used for treating the case
of idempotent and stabilisation nodes in the proof of
Lemma~\ref{lemma:over-computation-decomposition}.
\begin{lemma}\mylabel{lemma:conjugacy}
There exists a polynomial $\beta$ such that,
if $x_1,y_1,x_2,y_2\dots,x_m,y_m$ ($m\geq 1$) are elements of $M$
and $e$ is an idempotent
such that $x_h\cdot y_h\leq e$ for all $h=1\dots m$,
then $(y_1\cdot x_2)(y_2\cdot x_3)\cdots (y_{m-1}\cdot x_m)$
$n$-evaluates to $z$ such that:
\begin{itemize}
\item $x_1\cdot z\cdot y_m\leq e$, and;
\item if $m>\beta(n)$ or $(x_h\cdot y_h)\leq e^\sharp$ for some $h=1\dots m$ then $x_1\cdot z\cdot y_m\leq e^\sharp$.
\end{itemize}
\end{lemma}
\begin{proof}
Let us treat first the case $m\leq\beta(n)$, whatever is $\beta$.
Remark first that $(y_1\cdot x_2)\dots (y_{m-1}\cdot x_m)$
naturally $n$-evaluates to $z=\pi(y_1x_2\dots y_{m-1}x_m)$.
Thus $x_1\cdot z\cdot y_m=\pi(x_1y_1\cdots x_my_m)=e$.

Assume now that $m>\beta(n)$ for $\beta(n)=(n+K)^{3|M|}+1$
where $K$ is the constant obtained from Lemma~\ref{lemma:ordered-consistency}.
Set $d_i=(y_i\cdot x_{i+1})$ for all $i=1\dots m-1$.

We first claim ($\star$) that there exists $i<j$ such that $v=d_i\dots d_{j-1}$
$n$-evaluates to $y_i\cdot e^\sharp\cdot  x_j$.
For this, consider the word $u=d_1\dots d_{m-1}$,
and apply Theorem~\ref{theorem:exists-computation}
for producing an $(n+K)$-computation $U$ for $u$ of height at most $3|M|$.
The word $u$ has length $m-1>\beta(n)-1=(n+K)^{3|M|}$.
Thus there is a stabilisation node in $T$, say of degree $k>n+K$.
Let $S$ be a subtree of $T$ rooted at some stabilisation node.
Let $f$ be the (idempotent) value of the children of this node, the value of $S$ being $f^\sharp$.
This subtree corresponds to the factor $v=d_i\dots d_{j-1}$ of $u$.
We have to show that $v$ $n$-evaluates to $y_i\cdot e^\sharp\cdot x_j$.
The computation $S$ decomposes $v$ into $v_1,\dots, v_k$
and  each $v_h$ is of the form $d_{i_h}\dots d_{i_{h+1}-1}$
for some $h=1\dots k$ with $i=i_1<\dots<i_{k+1}=j$.
Define now $a_h$ to be $y_{i_h}$ and $b_h$ to be $\pi(x_{i_h+1} y_{i_h+1} \dots y_{i_{h+1}-1}x_{i_{h+1}})$
for all $h=1\dots k$. It is clear that $f\leq \pi(v_h)= a_h\cdot b_h$ for all $h=1\dots k$
since there is a computation over $v_h$ of value $f$.
Furthermore, $b_h\cdot a_{h+1}\leq e$ for all $h=1\dots k-1$.
Hence we can apply Lemma~\ref{lemma:ordered-consistency}, and get
that $f^\sharp\leq a_1\cdot e^\sharp\cdot b_k$.
Since furthermore $a_1=y_i$, and $b_k$ is either $\leq x_j$ or $\leq e\cdot x_j$,
it follows that $v$ $n$-evaluates to $f^\sharp\leq y_i\cdot e^\sharp\cdot x_j$.
This concludes the proof of the claim~($\star$).

Set now
$$z=\pi(y_1\dots y_i)\cdot e^\sharp\cdot \pi(x_j\dots y_m)\ .$$
Since, using the claim ($\star$), $d_1\dots d_{i-1}$, $d_i\dots d_{j-1}$, $d_j\dots d_{m-1}$
$n$-evaluate to $\pi(d_1\dots d_{i-1})$, $y_i\cdot e^\sharp\cdot x_j$,
	$\pi(d_j\dots d_{m-1})$, we get that $d_1\dots d_{m-1}$ $n$-evaluates to $z$.
Furthermore, $x_1\cdot z\cdot y_m=\pi(x_1\dots y_i)\cdot e^\sharp\cdot \pi(x_j\dots y_m)=e^\sharp$.
This proves the second conclusion of the statement.
\end{proof}

We are now ready to conclude.
\begin{proof}[Proof of Lemma~\ref{lemma:over-computation-decomposition}]
Let us set $\alpha(n)$ to be $(n+1)\beta(n)-1$,
where $\beta$ is the polynomial taken from Lemma~\ref{lemma:conjugacy}.
Lemma~\ref{lemma:over-computation-decomposition} follows from the following induction hypothesis:
\medskip

\noindent
{\em Induction hypothesis:} For all words
$u$ which $\alpha(n)$-evaluate to $b$,
and all decompositions of $u$ into $u_1,\dots,u_k$ ($k\geq 2$),
then $u_1,\dots,u_k$ $n$-evaluate to $b_1,\dots, b_k$,
and $b_2\dots b_{k-1}$ $n$-evaluate to $c$ such that $b_1\cdot c \cdot b_k\leq b$.

\noindent
{\em Induction parameter:} The height of the $\alpha(n)$-over-computation $T$
witnessing that  $\alpha(n)$-evaluates to $b$.
\medskip

It should be clear that this implies Lemma~\ref{lemma:over-computation-decomposition}
since this means that $b_1\dots b_k$ $n$-evaluate to $b_1\cdot c\cdot b_k\leq b$.

The essential idea in the proof of the induction hypothesis is that $T$
decomposes the word into $v_1,\dots,v_\ell$, and we have to study all
the possible ways the $v_i$'s and the $u_j$'s may overlap.
In practice, we will not refer much to $T$,
but simply about how it decomposes the word into $v_1,\dots,v_\ell$.
Thus, from now on, let $v_1,\dots,v_\ell$ and $u_1,\dots,u_k$ be decompositions of a word $u$
such that each of the $v_i$'s $\alpha(n)$-evaluates to $a_i$
and is subject to the application of the induction hypothesis.
\medskip 

\noindent
{\em Leaves.} This means that $\ell=1$. All the $u_h$'s should be empty, but one, say $u_h=a$
where $a$ is the letter labelling the leaf.
Three cases can occur depending on $h$. If $h=1$, then $u_1,\dots,u_k$ obviously $n$-evaluate
to $a,1,\dots,1,1$, and $1\dots1$ $n$-evaluate to $1$, and we indeed have $a\cdot 1\cdot 1\leq a$.
The case $h=k$ is symmetric. Finally, if $1<h<k$, then $u_1,\dots,u_k$ $n$-evaluate
to $1,\dots,1,a,1,\dots,1$, and $1\dots 1a1\dots 1$ $n$-evaluate to $a$, and we indeed have
$1\cdot a\cdot 1\leq a$.
\medskip

\noindent
{\em Binary nodes.}
If $\ell=2$, then there exist $s$ in $1,\dots, k$ and words $w,w'$ such that
\begin{align*}
v_1&=u_1\dots u_{s-1}w\ ,&
u_s&=ww'\ , &\text{and}\quad v_2&=w'u_{s+1}\dots u_k\ .
\end{align*}
We can apply the induction hypothesis to both $v_1$ and $v_2$.
We obtain that $u_1,\dots, u_{s-1},w$, $w',u_{s+1},\dots, u_k$ $n$-evaluate to
$b_1,\dots,b_{s-1},d,d',b_{s+1},\dots, b_k$,
and that $b_2\dots b_{s-1},b_{s+1}\dots b_k$ $n$-evaluate to $c_1,c_2$
such that $b_1\cdot c_1\cdot d\leq a_1$ and $d'\cdot c_2\cdot b_k\leq a_2$.
It follows that $u_s$ $n$-evaluates to $b_s=d\cdot d'$.
Furthermore, $b_2\dots b_{k-1}$ $n$-evaluates to $c_1\cdot b_s\cdot c_2=c$.
Overall, $u_1,\dots,u_k$ $n$-evaluate to $b_1,\dots,b_k$
and $b_2\dots b_{k-1}$ $n$-evaluates to $c$ such that $b_1\cdot c\cdot b_k=(b_1\cdot c_1\cdot d)\cdot(d'\cdot d_2\cdot b_k)\leq a_1\cdot a_2$.
\medskip

\noindent
{\em Idempotent and stabilisation nodes.}
Assume now that $v_1,\dots,v_\ell$ $\alpha(n)$-evaluate to $e,\dots,e$,
where $e$ is idempotent.
We aim at proving that $u_1,\dots,u_k$ $n$-evaluates to $b_1,\dots,b_k$,
and $b_2\dots b_{k-1}$ to $c$ such that $b_1\cdot c\cdot b_k\leq e$,
and if $\ell>\alpha(n)$, $b_1\cdot c\cdot b_k\leq e^\sharp$.


We rely on a suitable decomposition of the words:
there exist $0=i_0< i_1<\dots<i_m<i_{m+1}=\ell+1$ and $1=j_0<\dots<j_m=k$, as well as words
$\varepsilon=u'_0,u''_0,u'_1,u''_1,\dots,u'_m,u''_m=\varepsilon$ such that
\begin{align*}
v_{i_h}&=u''_{h-1}\,u_{j_{h-1}+1}\dots u_{j_{h}-1}\,u'_{h}&&
\text{for all $h=1\dots m$,}\tag{$\star$}\\
\text{and}\qquad
u_{j_h}&=u'_h\,v_{i_h+1}\dots v_{i_{h+1}-1}\,u''_h&&
\text{for all $h=0\dots m$.}\tag{$\star\star$}
\end{align*}
The best is to present it through a drawing. It is
annotated with all the variables that will be used during the proof.
The two main rows represent the two possible decompositions of the
word into $v_i$'s and $u_j$'s.
\begin{center}
\includegraphics[scale=1]{./lemma-comparison.pdf}
\end{center}
Such a decomposition is not unique. It is sufficient to guarantee that each separation
between some $u_s$ and some $u_{s+1}$ fall in some $v_{i_h}$, and that
each $v_{i_h}$ contains such a separation.

We can apply the induction hypothesis on each equation $(\star\star)$.
Hence, it follows that
$u''_{h-1},u_{j_{h-1}+1},\dots, u_{j_{h}-1},u'_{h}$ $n$-evaluate to $b''_{h-1},b_{j_{h-1}+1},\dots, b_{j_{h}-1},b'_{h}$
and $b_{j_{h-1}+1} \dots b_{j_{h}-1}$ $n$-evaluates to $c_h$, such that
$b''_{h-1}\cdot c_h\cdot b'_{h}\leq e$.
Set furthermore $b'_0=b''_m=1$. We get that $u'_h,u''_h$ $n$-valuate to $b'_h,b''_h$ for all $h=0\dots m$.
Define furthermore for all $h=0\dots m$, $e_h$ as
\begin{align*}
e_h&=\begin{cases}
		1&\text{if}~i_{h+1}-i_h-1=0\\
		e&\text{if}~1\leq i_{h+1}-i_h-1\leq n\\
		e^\sharp&\text{if}~i_{h+1}-i_h-1> n
		\end{cases}
\end{align*}
Since each $v_h$ $\alpha(n)$-evauates to $e$, each $v_h$ also $n$-evaluates to $e$.
Now $e_h$ has been chosen such that $v_{i_h+1}\dots v_{i_{h+1}-1}$
$n$-evaluates to $e_h$. Thus from $(\star\star)$, $u_{j_h}$
$n$-evaluates for all $h=0\dots m$ to $b_{j_h}$ that we define
as $b_{j_h}=b'_h\cdot e_h\cdot b''_h$.
At this point, we have that
\begin{asparadesc}
\item[C1] $u_1,\dots,u_k$ $n$-evaluate to $b_1,\dots,b_k$.
\end{asparadesc}

To head toward the conclusion, we will use Lemma~\ref{lemma:conjugacy}.
Thus, let us set $x_{h}$ to be $b''_{h-1}$  and $y_{h}$ to be $c_h\cdot b'_h\cdot e_h$ for all $h=1\dots m$.
We have
\begin{align*}
x_h\cdot y_h&=(b''_{h-1}\cdot c_h\cdot b'_h)\cdot e_h=e\cdot e_h . \tag{$\dagger$}
\end{align*}
According to ($\dagger$), $x_h\cdot y_h\leq e$, and we can apply Lemma~\ref{lemma:conjugacy} to 
\begin{align*}
x_1,y_1,x_2,\dots, x_m,y_m
\end{align*}
and obtain that $(y_1\cdot x_2)\dots (y_{m-1}\cdot x_m )$ $n$-evaluates to some $z$
subject to the conclusions of the lemma (we will recall these conclusions upon need).

Let us now establish the following claims C2, C3 and C4.
\begin{asparadesc}
\item[C2] $b_2 \dots b_{k-1}$ $n$-evaluates to $(z\cdot c_m)$.\\
	Indeed, for all $h=1\dots m$, $c_h$ is chosen such that
	$b_{j_{h-1}+1} \dots b_{j_{h}-1}$ $n$-evaluates to $c_h$, thus
	$b_{j_{h-1}+1} \dots b_{j_{h}}$ $n$-evaluates to:
	\begin{align*}
	c_h\cdot b_{j_h}&=c_h\cdot b'_h\cdot e_h\cdot b''_h= y_h\cdot x_{h+1}\ ,
	\end{align*}
	by just unfolding the definitions. Since furthermore $(y_1\cdot x_2)\dots (y_{m-1}\cdot x_m )$ $n$-evaluates to $z$,
	it follows that $b_2\dots b_{j_{m-1}}$ $n$-evaluates to $z$.
	Furthermore, by choice of $c_m$, $b_{j_{m-1}+1}\dots b_{k-1}$ $n$-evaluates to $c_m$.
	Thus $b_2\dots b_{k-1}$ $n$-evaluates to $(z\cdot c_m)$ as claimed.
\item[C3] $b_1\cdot (z\cdot c_m) \cdot b_k\leq e$. \\
	Indeed, according to the conclusions of Lemma~\ref{lemma:conjugacy},
	$x_1\cdot z\cdot y_m\leq e$. Hence,
	\begin{align*}
	b_1\cdot (z\cdot c_m)\cdot b_k&=e_0\cdot x_1\cdot z \cdot y_m\leq e_0\cdot e\leq e\ . 
	\end{align*}
\item[C4] if $\ell>\alpha(n)=(n+1)\beta(n)-1$ then $b_1\cdot (z\cdot c_m) \cdot b_k\leq e^\sharp$
	(with $\beta$ taken from Lemma~\ref{lemma:conjugacy}).\\
	Since $i_0=0$ and $i_{m+1}=\ell+1$, we have
		$$\ell=m+\sum_{h=0}^m(i_{h+1}-i_h-1).$$
	Since $\ell>(n+1)\beta(n)-1$ this means that either $m>\beta(n)$,
	or $i_{h+1}-i_h-1>n$ for some $h=0\dots m$.
	This means that either $m>\beta(n)$, or $e_h=e^\sharp$ for some $h=0\dots m$.
	In all cases, 
	\begin{align*}
	b_1\cdot (z\cdot c_m)\cdot b_k&=e_0\cdot x_1\cdot z \cdot y_m\leq e^\sharp\ . 
	\end{align*}
	The last inequality can have three origins. Either $m>\beta(n)$ or $e_h=e^\sharp$
	(recall ($\dagger$) stating that $x_h\cdot y_h\leq e\cdot e_h$)
	for some $h=1\dots m$, or $e_0=e^\sharp$. In the two first cases, by Lemma~\ref{lemma:conjugacy},
	$x_1\cdot 	z\cdot y_m\leq e^\sharp$, and thus $e_0\cdot x_1\cdot z\cdot y_m\leq e^\sharp$
	(since $e_0$ is either $1$, or $e$, or $e^\sharp$).
	In the third case,
	$e_0\cdot x_1\cdot z\cdot  y_m\leq e^\sharp$ since $x_1\cdot z\cdot y_m\leq e$.
\end{asparadesc}

Gathering the claims C1, C2, C3,
we get that $u_1,\dots,u_k$ $n$-evaluate to $b_1,\dots,b_k$,
that $b_2\dots b_{k-1}$ $n$-evaluates to $c=z\cdot c_m$ and that $b_1\cdot c\cdot b_k\leq e$.
This is exactly the induction hypothesis for the idempotent node case.
If we further gather C4, we get that if the root node of $T$ is a stabilisation node, 
$b_1\cdot c\cdot b_k\leq e$. Once more the induction hypothesis is satisfied.
\end{proof}









==> msocard.tex <==
% !TEX root =  stabilisation_monoids_v4_final.tex

\section{Logic}
\label{section:logic}

\subsection{Cost monadic logic}

Let us recall that monadic second-order logic (monadic logic for short)
is the extension of first-order logic with the ability to quantify over
sets ({\it i.e.}, monadic relations). 
Formally monadic formulae use \intro{first-order variables} ($x,y,\dots$),
and \intro{monadic variables} ($X,Y,\dots$), and it is allowed in
such formulae to quantify existentially and universally over both
first-order and monadic variables, to use every boolean connective, 
to use the membership predicate ($x\in X$),
and every predicate of the relational structure.
%It is classical that over words (finite or infinite) as well as trees (finite or infinite),
%the expressiveness of monadic logic coincide with standard form of automata.
We expect from the reader basic knowledge concerning monadic logic.
\begin{example}\label{example:MSO}
The monadic formula~$\mathtt{reach}(x,y,X)$ over the signature containing the single binary predicate $\mathbf{edge}$ (signature of a digraph):
\begin{multline*}
\mathtt{reach}(x,y,X)::=\quad x=y\quad\vee\quad\forall Z\\
	\left(x\in Z\wedge\forall z,z'~(z\in Z\wedge z'\in X\wedge \mathbf{edge}(z,z')\rightarrow z'\in Z)\right)
		\quad\rightarrow\quad y\in Z
\end{multline*}
describes the existence of a path in a digraph from vertex~$x$ to vertex~$y$ such that
all edges appearing in the path end in~$X$.
Indeed, it expresses that either the path is empty, or every sets~$Z$ containing~$x$
and closed under taking edges ending in~$X$, also contains~$y$.
\end{example}

In \intro{cost monadic logic},
one uses a single extra variable~$N$ of a new kind, called the
\intro{bound variable}. It ranges over non-negative integers.
\intro {Cost monadic} logic is obtained from monadic logic by allowing the extra predicate $|X|\leq N$ -- in which $X$
is some monadic variable and $N$ the bound variable -- if and only if it appears \emph{positively} in the formula
({\it i.e.}, under the scope of an even number of negations).
The semantic of~$|X|\leq N$ is, as one may expect, to be
satisfied if (the valuation of) $X$ has cardinality at most (the valuation of) $N$. 
Given a formula~$\varphi$, we denote by~$\FV(\varphi)$ its free variables, the bound variable excluded.
A formula that has no free-variables--it may still use the bound variable--is called a \intro{sentence}.

We now have to provide a meaning to the formulae of cost monadic logic.
We assume some familiarity of the reader with logic terminology.
A \intro{signature} consists of a set of symbols~$R,S,\dots$. To each symbol is attached
a non-negative integer called its \intro{arity}.
A (relational) \intro{structure} (over the above signature)
$\structure=\langle U_\structure,R^\structure,\dots,R^\structure\rangle$ consists of a set~$U_\structure$
called the \intro{universe}, and for each symbol~$R$ of arity~$n$ of a
relation~$R^\structure\subseteq U_\structure^n$.
Given a set of variables~$F$, a valuation of~$F$ (over~$\structure$)
is a mapping~$\valuation$ which to each monadic variable~$X\in F$
associates a set~$\valuation(X)\subseteq U_\structure$, and to each
first-order variable~$x\in F$ associates an element~$\valuation(x)\in U_\structure$.
We denote by~$\valuation,X=E$ the valuation~$\valuation$ in which~$X$ is further mapped to~$E$.
Given a cost monadic formula~$\varphi$, a valuation~$\valuation$ of its free variable over a structure~$\structure$
and a non-negative integer~$n$,
we express by $\structure,\valuation,n\models\varphi$ the fact that the formula~$\varphi$
is satisfied over the structure~$\structure$ with valuation~$\valuation$ when the variable~$N$ takes the value~$n$.
Of course, if~$\varphi$ is simply a sentence, we just write~$\structure,n\models\varphi$.
We also omit the parameter~$n$ when~$\varphi$ is a monadic formula.

The positivity assumption required when using the predicate~$|X|\leq N$ has straightforward
consequences.
Namely, for all cost monadic sentences $\varphi$, all relational structures~$\structure$,
and all valuations~$\valuation$,
$\structure,\valuation,n\models\varphi$ implies $\structure,\valuation,m\models\varphi$ for all~$m\geq n$.

Instead of evaluating as true or false as done above,
we see a formula of cost monadic logic~$\varphi$ of free variables~$F$
as associating to each relational structure~$\structure$ and each valuation~$\valuation$ 
of the free variables a value in~$\NI$ defined by:
$$
\sem{\varphi}(\structure,\valuation)=\inf\{n~:~\structure,\valuation,n\models\varphi\}\ .
$$
This value can be either a non-negative integer, or~$\infty$ if no valuation of~$N$
makes the sentence true.
In case of a sentence~$\varphi$, we omit the valuation and simply write~$\sem\varphi(\structure)$.
Let us stress the link with standard monadic logic in the following fact:
\begin{myfact}
For all monadic formula~$\varphi$, and all relational structures~$\structure$,
\begin{align*}
\sem\varphi(\structure)&=\begin{cases}
	0&\text{if}~\structure\models\varphi\\
	\infty&\text{otherwise\ .}
	\end{cases}
\end{align*}
\end{myfact}

\begin{example}\label{example:MSOc}
The sentence $\forall X~|X|\leq N$ calculates the
size of a structure. More formally $\sem{\forall X~|X|\leq N}(\structure)$
equals $|U_\structure|$.

A more interesting example makes use of Example~\ref{example:MSO}.
Again over the signature of digraphs, the cost monadic sentence:
$$
\mathtt{diameter}::=\forall x,y~\exists X~|X|\leq N\wedge\mathtt{reach(x,y,X)}.
$$
defines the diameter of the di-graph: indeed, the diameter of a graph is the least~$n$
such that for all pairs of states~$x,y$, there exists a set of size at most~$n$
allowing to reach $y$ from~$x$ (recall that in the definition of~$\mathtt{reach}(x,y,X)$,
$x$ does not necessarily belong to~$X$, hence this is the diameter in the standard sense).
\end{example}

From now on, for avoiding some irrelevant considerations, we will consider the variant of
cost monadic logic in which a) only monadic variables are allowed,
b) the inclusion relation $X\subseteq Y$ is allowed, and c) each relation over elements is
raised to a relation over singleton sets.
Keeping in mind that each element can be identified with the unique singleton set containing
it, it is easy to translate cost monadic logic into this variant.
In this presentation, it is also natural to see the inclusion relation as any other relation.
We will also assume that the negations are pushed to the leaves of formulae as is usual.
Overall a formula can be of one of the following forms:
$$
R(X_1,\dots X_n)\quad|\quad\neg R(X_1,\dots X_n)\quad|\quad|X|\leq N\quad|\quad\varphi\wedge\psi\quad|\quad\varphi\vee\psi\quad|\quad 
	\exists X.\varphi\quad|\quad\forall X.\varphi
$$
in which~$\varphi$ and~$\psi$ are formulas, $R$ is some symbol of arity~$n$ which can possibly be~$\subseteq$
(of arity~$2$), and~$X,X_1,\dots,X_n$ are monadic variables.

So far, we have described the semantic of cost monadic logic from the standard notion of model.
There is another equivalent way to describe the meaning of formulae, by induction
on the structure.
The equations are disclosed in the following fact.
\begin{myfact}\label{fact:induction-logic}
Over a structure~$\structure$ and a valuation~$\valuation$, the following equalities hold:
\begin{align*}
\sem{R(X_1,\dots,X_n)}(\structure,\valuation)		&=\begin{cases}0 & \text{if}~R^\structure(\valuation(X_1),\dots,\valuation(X_n))\\
												\infty&\text{otherwise}\end{cases}\\
\sem{\neg R(X_1,\dots,X_n)}(\structure,\valuation)	&=\begin{cases}\infty & \text{if}~R^\structure(\valuation(X_1),\dots,\valuation(X_n))\\
												0&\text{otherwise}\end{cases}\\
\sem{|X|\leq N}(\structure,\valuation)				&=|\valuation(X)|\\
\sem{\varphi\vee\psi}(\structure,\valuation)			&=\min(\sem\varphi(\structure,\valuation),\sem\psi(\structure,\valuation))\\
\sem{\varphi\wedge\psi}(\structure,\valuation)		&=\max(\sem\varphi(\structure,\valuation),\sem\psi(\structure,\valuation))\\
\sem{\exists X~\varphi}(\structure,\valuation)			&=\inf\{\sem\varphi(\structure,\valuation,X=E)~:~E\subseteq U_\structure\}\\
\sem{\forall X~\varphi}(\structure,\valuation)			&=\sup\{\sem\varphi(\structure,\valuation,X=E)~:~E\subseteq U_\structure\}
\end{align*}
\end{myfact}

As it is the case for monadic logic, no property (if not trivial) is decidable for monadic logic in general.
Since cost monadic logic is an extension of monadic logic, one cannot expect anything to be
better in this framework.
However we are interested, as in the standard setting, to decide properties over a restricted class
$\mathcal{C}$ of structures. The class~$\mathcal C$ can typically be the class of
finite words, of finite trees, of infinite words (of length~$\omega$, or beyond) or of infinite trees.
The subject of this paper is to consider the case of finite words over a fixed finite alphabet.

We are interested in deciding properties concerning the function described by cost monadic formulae
over~$\mathcal C$. But what kind of properties?
It is quite easy to see that, given a cost monadic sentence~$\varphi$ and~$n\in\nats$,
one can effectively produce a monadic formula~$\varphi^n$ such that for all
structures~$\structure$,
$\structure\models\varphi^n$ iff $\sem\varphi(\structure)=n$ (such a translation
would be possible even without assuming the positivity requirement in the use of the
predicates $|X|\leq N$).
Hence, deciding questions of the form~``$\sem\varphi=n$'' can be reduced to the
standard theory.

Properties that cannot be reduced to the standard theory, and that we are
interested in, involve the existence of bounds. One says below that a function
$f$ is \intro{bounded over} some set~$X$ if there is some 
integer~$n$ such that~$f(x)\leq n$
for all~$x\in X$. We are interested in the following generic problems:
\begin{description}	
\item[Boundedness] Is the function~$\sem\varphi$ bounded over~$\mathcal{C}$?\\
	Or (variant), is~$\sem\varphi$ bounded over a regular subset of~$\mathcal{C}$?\\
	Or (limitedness),  is~$\sem\varphi$ bounded over~$\{\structure~:~\sem{\varphi}(\structure)\neq\infty\}$?
\item[Divergence] For all~$n$, do only finitely many~$\structure\in\mathcal{C}$ satisfy~$\sem\varphi(\structure)\leq n$?
	\\Said differently, are all sets over which~$\sem\varphi$ is bounded of finite
	cardinality?
%	\\Or, does there exist~$n\in\infty$ such that infinitely many $\structure\in\mathcal{C}$ do satisfy~$\sem\varphi(\structure)\leq n$?
\item[Domination] For all~$E\subseteq\mathcal{C}$, does $\sem\varphi$ bounded over~$E$ imply that $\sem\psi$
	is also bounded over~$E$?
%	Or, does there exist a subset~$E\subseteq\mathcal{C}$ such that~$\sem\varphi$ is bounded over~$E$ while~$\sem\psi$
%	is not?
\end{description}
All these questions cannot be reduced (at least simply) to questions in the standard theory.
Furthermore, all these questions become undecidable for very standard reasons as
soon as the requirement of positivity in the use of the new predicate~$|X|\leq N$ is removed.
In this paper, we introduce suitable material for proving their
decidability over the class~$\mathcal C$ of words.

 One easily sees that the domination question is in fact a joint extension of the boundedness question
(if one sets $\varphi$ to be always true, {\it i.e.}, to compute the constant function~$0$),
and the divergence question (if one sets~$\psi$ to be measuring the size of the structure,
{\it i.e.}, $\forall X~|X|\leq N$).
Let us remark finally that if~$\varphi$ is a formula of monadic logic, then the boundedness question
corresponds to deciding if~$\varphi$ is a tautology. If furthermore~$\psi$ is also monadic, then the domination
consists of deciding whether~$\varphi$ implies~$\psi$.

In the following section, we introduce the notion of cost functions, {\it i.e.}, equivalence classes
over functions allowing to omit discrepancies of the function described, while preserving
sufficient information for working with the above questions.

\subsection{Cost functions}
\label{subsection:cost-function}

In this section, we introduce the equivalence relation~$\approx$ over functions,
and the central notion of cost function.

A \intro{correction function} $\alpha$ is a non-decreasing mapping from~$\nats$ to~$\nats$
such that~$\alpha(n)\geq n$ for all~$n$.
From now on, the symbols $\alpha,$ $\alpha'\dots$ implicitly designate correction functions.
Given $x,y$ in~$\NI$, $x\preccurlyeq_\alpha y$
holds if~$x\leq \overline\alpha(y)$ in which~$\overline\alpha$ is the extension of~$\alpha$
with~$\overline\alpha(\infty)=\infty$. For every set~$E$, $\preccurlyeq_\alpha$
is extended to~$(\NI)^E$ in a natural way by~$f \preccurlyeq_\alpha g$
if $f(x)\preccurlyeq_\alpha g(x)$ for all~$x\in E$, or equivalently $f\leq\overline\alpha \circ g$.
Intuitively, $f$ is dominated by~$g$ after it has been ``stretched''
by~$\alpha$.
One also writes $f\approx_\alpha g$ if~$f\preccurlyeq_\alpha g$ and~$g\preccurlyeq_\alpha f$.
Finally, one writes $f \preccurlyeq g$ (resp. $f\approx g$) if~$f\preccurlyeq_\alpha g$
(resp. $f\approx_\alpha g$) for some~$\alpha$.
A \intro{cost function} (over a set~$E$) is an equivalence class of~$\approx$
({\it i.e.}, a set of mappings from~$E$ to~$\NI$).


Some elementary properties of~$\preccurlyeq_\alpha$ are:
\begin{myfact}\label{fact:preccurlyeq-elem}
If~$\alpha\leq\alpha'$ and~$f\preccurlyeq_\alpha g$, then~$f\preccurlyeq_{\alpha'} g$.
If~$f\preccurlyeq_\alpha g\preccurlyeq_{\alpha'} h$, then $f\preccurlyeq_{\alpha\circ\alpha'} h$.
\end{myfact}
The above fact allows to work with a single correction function at a time. 
Indeed, as soon as two correction functions~$\alpha$ and~$\alpha'$ are involved in the same proof,
we can consider the correction function~$\alpha''=\max(\alpha,\alpha')$. By the above fact,
it satisfies that $f\preccurlyeq_\alpha g$ implies~$f\preccurlyeq_{\alpha''} g$,
and~$f\preccurlyeq_{\alpha'} g$ implies~$f\preccurlyeq_{\alpha''} g$.

\begin{example}\label{example:approx}
Over~$\nats\times\nats$, maximum and sum are equivalent for the doubling correction function (for short, $(\max)\approx_{\times2}(+)$). 
Indeed, for all~$x,y\in\omega$,
$$\max(x,y)\leq x+y\leq 2\times\max(x,y)\ .$$

\noindent
Our next examples concern mappings from sequences of words to~$\nats$.
We have 
\begin{align*}
|~|_a&\preccurlyeq |~|\ ,&\text{and}\qquad|~|_a\not\preccurlyeq |~|_b\ ,
\end{align*}
where $a$ and $b$ are distinct letters, $|~|$ is the function mapping each word to its length
and $|~|_a$ the function mapping each word to the number of occurrences of the letter $a$ it contains.
Indeed we have $|~|_a\leq|~|$
but the set of words $a^*$ is a witness that $|~|_a\preccurlyeq_\alpha|~|_b$
cannot hold whatever is $\alpha$.

\noindent
Given words $u_1,\dots,u_k\in\{a,b\}^*$, we have
$$|u_1\dots u_k|_a\approx_\alpha \max(|K|,\max_{i=1\dots k}|u_i|_a)
\qquad\text{where}\quad K=\{i\in\{1,\dots,k\}~:~|u_i|_a\geq 1\}
$$
in which~$\alpha$ is the squaring function.
 Indeed, for one direction we just have to remark:
\begin{align*}
\max(|K|,\max_{i=1\dots k}|u_i|_a)&\leq |u_1\dots u_k|_a,
\end{align*}
and for the other direction we use:
\begin{align*}
|u_1\dots u_k|_a&\leq \sum_{i\in K}|u_i|_a\leq(\max(|K|,\max_{i=1\dots k}|u_i|_a))^2\ .
\end{align*}
\end{example}
The relation~$\preccurlyeq$ has other characterisations:
\begin{proposition}\label{proposition:preccurlyeq-characterisation}
For all $f,g$ from~$E$ to~$\NI$, the following items are equivalent:
\begin{enumerate}
\item $f\preccurlyeq g$, \label{item:dominiation-preccurly}
\item $\forall n\in\nats\ \exists m\in\nats\ \forall x\in E~g(x)\leq n\rightarrow f(x)\leq m\ ,$ and;\label{item:domination-quantif}
\item for all $X\subseteq E$, $g|_X$ is bounded implies $f|_X$ is bounded.\label{item:domination-bounded}
\end{enumerate}
\end{proposition}
\begin{proof}
\emph{From (\ref{item:dominiation-preccurly}) to (\ref{item:domination-quantif}).}
Let us assume $f\preccurlyeq g$, {\it i.e.}, $f\preccurlyeq_\alpha g$ for some~$\alpha$.
Let~$n$ be some non-negative integer, and~$m=\alpha(n)$.
We have for all~$x$, that~$g(x)\leq n$
implies~$f(x)\leq(\alpha\circ g)(x)\leq \alpha(n)=m$, thus establishing the second statement.

\emph{From (\ref{item:domination-quantif}) to (\ref{item:domination-bounded}).}
Let~$X\subseteq E$ be such that~$g|_X$ is bounded. Let~$n$ be a bound of~$g$ over~$X$.
Item~(\ref{item:domination-quantif}) states the existence of~$m$ such
that~$\forall x\in E\ g(x)\leq n\rightarrow f(x)\leq m$.
In particular, for all~$x\in E$, we have~$g(x)\leq n$ by choice of~$n$, and hence $f(x)\leq m$.
Hence~$f|_X$ is bounded by~$m$.

\emph{From (\ref{item:domination-bounded}) to (\ref{item:dominiation-preccurly}).}
Let~$n\in\nats$, consider the set~$X_n=\{x~:~g(x)\leq n\}$.
The mapping $g$ is bounded over~$X_n$ (by~$n$), and hence by (\ref{item:domination-bounded}), $f$ is also bounded.
We set~$\alpha(n)=\max(n,\sup f(X_n))$. Since $X_n\subseteq X_{n+1}$, the  function~$\alpha$
is non-decreasing. Since furthermore~$\alpha(n)\geq n$, $\alpha$ is a correction function.
Let now~$x\in X$. If~$g(x)<\infty$, we have that~$x\in X_{g(x)}$ by definition of the $X$'s.
Hence~$f(x)\leq\sup f(X_{g(x)})=\alpha(g(x))$. 
Otherwise~$g(x)=\infty$, and we have~$f(x)\leq\overline\alpha(g(x))=\infty$.
Hence~$f\preccurlyeq_\alpha g$.
\end{proof}

The last characterisation shows that the relation~$\approx$
is an equivalence relation that preserves the existence of bounds.
Indeed, all this theory can be seen as a method for
proving the existence/non-existence of bounds.
One can also remark that the questions of boundedness, divergence,
and domination presented in the previous section,
are preserved under replacing the semantic of a formula
by an~$\approx$-equivalent function. Furthermore, the domination question
can be simply reformulated as~$\sem\varphi\succcurlyeq\sem\psi$.

We conclude this section by some remarks on the structure of the $\preccurlyeq$ relation.
Cost functions over some set~$E$  ordered by~$\preccurlyeq$  form a lattice.
Let us show how this lattice refines the lattice of subsets of~$E$ ordered by inclusion.
The following elementary fact shows that we can identify a subset of~$E$
with the cost function of its characteristic function
(given a subset~$X\subseteq E$, one denotes by~\intro{$\chi$}$_X$
its \intro{characteristic mapping} defined by~$\chi_X(x)=0$ if~$x\in X$, and $\infty$ otherwise):
\begin{myfact}
For all $X,Y\subseteq E$, $\chi_X\preccurlyeq\chi_Y$ iff $X\supseteq Y$.
\end{myfact}
In this respect, the lattice of cost functions is a refinement of the lattice of subsets
of~$E$ equipped with the superset ordering. Let us show that this refinement is strict.
Indeed, there is only one language~$L$ such that~$\chi_L$
does not have~$\infty$ in its range, namely~$L=E$, however, we will
show in Proposition~\ref{proposition:cost-functions-uncountable}
that, as soon as $E$ is infinite, there are uncountably many cost functions
which have this property of not using the value~$\infty$.
\begin{proposition}\label{proposition:cost-functions-uncountable}
If~$E$ is infinite, then there exist at least continuum many different cost functions from~$E$ to~$\nats$.
\end{proposition}
\begin{proof}
Without loss of generality, we can assume $E$ countable, and even, up
to bijection, that $E=\nats\setminus\{0\}$.
Let~$p_0,p_1,\dots$ be the sequence of all prime numbers. Every $n\in E$
is decomposed in a unique way as~$p_1^{n_1}p_2^{n_2}\dots$ in which all~$n_i$'s
are null but finitely many (with an obvious meaning of the infinite product).
For all~$I\subseteq\nats$, one defines the function~$f_I$ from~$\nats\setminus\{0\}$ to~$\nats$
for all~$n\in\nats\setminus\{0\}$ by:
\begin{align*}
f_I(n)&=\max\{n_i~:~i\in I,~n=p_1^{n_1}p_2^{n_2}\dots\}\ .
\end{align*}
Consider now two different sets~$I,J\subseteq\nats$.
This means---up to a possible exchange of the roles of~$I$ and~$J$---that there exists~$i\in I\setminus J$.
Consider now the set~$X=\{p_i^k~:~k\in\nats\}$.
Then, by construction,~$f_I(p_i^k)=k$ and hence~$f_I$ is not bounded over~$X$.
However, $f_J(p_i^k)=0$ and hence~$f_J$ is bounded over~$X$.
It follows by Proposition~\ref{proposition:preccurlyeq-characterisation} that~$f_I$ and~$f_J$
are not equivalent for~$\approx$. We can finally conclude that---since there exist continuum many subsets of~$\nats$---
there is at least continuum many cost functions over~$E$ which do not use value $\infty$.
\end{proof}

%TODO usefulness of fact:sim-inf-sup

%Let us complete this section with the following convenient fact:
%\begin{myfact}\label{fact:sim-inf-sup}
%For all sets~$E,F\subseteq\nats$, and all correction function~$\alpha$, we have;
%\begin{align*}
%\inf E&\preccurlyeq_\alpha\inf F&\text{iff}\quad&\forall n\in F.\,\exists m\in E.~m\leq\alpha(n)\ ,\\
%\sup E&\preccurlyeq_\alpha\sup F&\text{iff}\quad&\forall m\in E.\,\exists n\in F.~m\leq\alpha(n)\ ,\\
%\text{and}\qquad
%\sup E&\preccurlyeq_\alpha\inf F&\text{iff}\quad&\forall m\in E.\,\forall n\in F.~m\leq \alpha(n)\ .
%\end{align*}
%\end{myfact}

\subsection{Solving cost monadic logic over words using cost functions}

As usual, we see a word as a structure, the universe of
which is the set of positions in the word (numbered from~$1$),
equipped with the ordering relation~$\leq$,
and with a unary relation for each letter of the alphabet that we interpret as the set of
positions at which the letter occur.
Given a set of monadic variables~$F$, and a valuation~$\valuation$ of~$F$
over a word~$u=a_1\dots a_k\in\alphabet^*$, we denote by~$\langle u,\valuation\rangle$
the word~$c_1\dots c_k$ over the alphabet~$\alphabet_F=\alphabet\times\{0,1\}^F$ such
that for all position~$i=1\dots k$, $c_i=(a_i,\delta_i)$
in which~$\delta_i$ maps~$X\in F$ to~$1$ if~$i\in\valuation(X)$,
and to $0$ otherwise.

It is classical that given a monadic formula~$\varphi$ with free variables~$F$, the language
$$
L_\varphi=\{\langle u,\valuation\rangle~:~u,\valuation\models\varphi\}\subseteq\alphabet_F^*
$$
is regular. The proof is done by induction on the formula.
It amounts to remark that to the constructions of the logic, namely
disjunction, conjunction, negation and existential quantification,
correspond naturally some language theoretic operations, namely union, intersection,
complementation and projection.
The base cases are obtained by remarking that the relations of ordering,
inclusion, and letter, also correspond to regular languages.

We use a similar approach. To each cost monadic formula~$\varphi$ with
free variables~$F$ over the signature of words over~$\alphabet$,
we associate the cost function~$f_\varphi$ over~$\alphabet_F$ defined by
$$
f_\varphi(\langle u,\valuation\rangle)=\sem\varphi(u,\valuation)\ .
$$
We aim at solving cost monadic logic by providing an explicit representation to the
cost functions $f_\varphi$.
For reaching this goal, we need to define a family
of cost functions~$\mathcal F$
that contains suitable constants, has effective closure properties
and decision procedures.

The first assumption we make is the closure under \intro{composition with a morphism}.
{\it I.e.}, let~$f$ be a cost function in~$\mathcal F$ over~$\alphabet^*$
and~$h$ be a morphism from~$\alphabetB^*$ ($\alphabetB$ being another alphabet)
to~$\alphabet^*$, we require~$f\circ h$ to also belong to~$\mathcal F$.
In particular, this operation allows us to change the alphabet, and hence to add
new variables when required. It corresponds to the closure under
inverse morphism for regular languages.

Fact~\ref{fact:induction-logic} gives us a very precise idea of the constants we need.
The constants correspond to the formulae of the form~$R(X_1,\dots,X_n)$ as well as their
negation. As mentioned above, for such a formula~$\varphi$, $L_\varphi$ is regular.
Hence, it is sufficient for us to require that the characteristic
function~$\chi_L$ belongs to~$\mathcal F$ for each regular language~$L$.
The remaining constants correspond to the formula~$|X|\leq N$.
We have that~$f_{|X|\leq N}(\langle u,X=E\rangle)=|E|$.
This corresponds to counting the number of occurrences of letters from~$\alphabet\times\{1\}$
in a word over~$\alphabet\times\{0,1\}$. Up to a change of alphabet (thanks to the closure under composition with a morphism)
it will be sufficient for us that~$\mathcal F$ contains
the function~``$\mathrm{size}$'' which maps each word~$u\in\{a,b\}^*$ to $|u|_a$.

Fact~\ref{fact:induction-logic} also gives us a very precise idea of the closure properties we need.
We need the closure under $\min$ and~$\max$ for disjunctions and conjunctions.
For dealing with existential and universal quantification, we need the new operations
of \intro{$\inf$-projection} and \intro{$\sup$-projection}.
Given a mapping $f$ from~$\alphabet^*$ to~$\NI$ and a mapping~$h$ from~$\alphabet$
to~$\mathbb{B}$ that we extend into a morphism from~$\alphabet^*$ to~$\mathbb{B}^*$
($\mathbb{B}$ being another alphabet)
the \intro{inf-projection} of~$f$ with respect to~$h$ is
the mapping $f_{\inf,h}$ from~$\mathbb{B}^*$ to~$\NI$ defined for all~$v\in\mathbb{B}^*$ by:
\begin{align*}
f_{\inf,h}(v)&=\inf\{f(u)~:~h(u)=v\}\ .
\end{align*}
Similarly, the \intro{sup-projection} of~$f$ with respect to~$h$ is
the mapping $f_{\sup,h}$ from~$\mathbb{B}^*$ to~$\NI$ defined for all~$v\in\mathbb{B}^*$ by:
\begin{align*}
f_{\sup,h}(v)&=\sup\{f(u)~:~h(u)=v\}\ .
\end{align*}

We summarise all the requirements in the following fact.
\begin{myfact}\label{fact:schema-cost-monadic}
Let~$\mathcal F$ be a class of cost functions  over words such that:
\begin{enumerate}
\item for all regular languages $L$, $\chi_L$ belongs to~$\mathcal F$, \label{item:F-reg}
\item $\mathcal F$ contains the cost function ``$\mathrm{size}$'',\label{item:F-size}
\item $\mathcal F$ is effectively closed under composition with a morphism, $\min$, $\max$, $\inf$-projection and $\sup$-projection,
	\label{item:F-closure}
\item $\preccurlyeq$ is decidable over~$\mathcal F$,
	\label{item:F-decidability}
\end{enumerate}
then the boundedness, divergence and domination problems are decidable for cost monadic logic over words.
\end{myfact}

%TODO adapt the end of section on cost MSO

The remainder of the paper is devoted to the introduction of the class of recognisable cost functions,
and showing that this class satisfies all the assumptions of Fact~\ref{fact:schema-cost-monadic}.
In particular, Item~\ref{item:F-reg} is established as Example~\ref{example:language-recognisable}.
Item~\ref{item:F-size} is achieved in Example~\ref{example:recognisable-size}.
Item~\ref{item:F-closure} is the subject of Fact~\ref{fact:recognisable-composition-morphism},
Corollary~\ref{corollary:rec-min-max} and
Theorems~\ref{theorem:inf-projection} and \ref{theorem:sup-projection}.
Finally, Item~\ref{item:F-decidability} is established in Theorem~\ref{theorem:rec-domination}.

Thus we deduce our main result.
\begin{theorem}\label{theorem:main}
The domination relation is decidable for cost-monadic logic over finite words.
\end{theorem}

All these results are established in Section~\ref{section:recognisability}.
However, we need first to introduce the notion of stabilisation monoids, as well as some of
its key properties. This is the subject of Section~\ref{section:stabilisation-monoid}.



==> recognisability.tex <==
% !TEX root =  stabilisation_monoids_v4_final.tex


\section{Recognisable cost functions}
\label{section:recognisability}

We have seen in the previous sections the notion of stabilisation monoids,
as well as the key technical tools for dealing with them, namely computations,
over-computations and under-computations.
In particular, we have seen Theorem~\ref{theorem:exists-computation}
and Theorem~\ref{theorem:unicity-computations} that state the existence
of computations and the ``unicity'' of their values.
In this section, we put these notions in action, and introduce the definition
of recognisable cost functions. We will see in particular that 
the hypothesis of Fact~\ref{fact:schema-cost-monadic}
is fulfilled by recognisable cost functions, and as a consequence
the domination problem for cost-monadic logic is decidable over finite
words.


\subsection{Recognisable cost functions}
\label{subsection:definition-recognisability}

Let us fix a stabilisation monoid $\monoid$.
An \intro{ideal} of~$\monoid$ is a subset~$I$ of~$M$ which is downward closed,
{\it i.e.}, such that whenever $a\leq b$ and $b\in I$ we have~$a\in I$.
Given a subset~$X\subseteq M$, we denote by~$X\ideal$
the least ideal which contains $X$, {\it i.e.}, $X\ideal=\{y~:~y\leq x,~x\in X\}$.

The three ingredients used for recognising a cost functions are
a monoid $\monoid$, a mapping~$h$ from letters of the alphabet $\alphabet$ to $M$
(that we extend into a morphism $\tilde h$ from $\alphabet^*$ to $M^*$),
and an ideal~$I$.

We then define for each non-negative integer~$p$ four functions from $\alphabet^*$ to $\NI$:
\begin{center}
\begin{tabular}{ll}
$\sem{\monoid,h,I}^{--}_p(u)$&= $\inf\{n~:~$there exists an $n$-under-computation of value in~$M\setminus I$\\
		&\qquad\qquad of height at most~$p$ for~$\tilde h(u)$ $\}$\\
$\sem{\monoid,h,I}^{-}_p(u)$&= $\inf\{n~:~$there exists an $n$-computation of value in~$M\setminus I$\\
		&\qquad\qquad of height at most~$p$ for~$\tilde h(u)$ $\}$\\
$\sem{\monoid,h,I}^{+}_p(u)$&= $\sup\{n+1~:~$there exists an $n$-computation of value in~$I$\\
		&\qquad\qquad of height at most~$p$ for~$\tilde h(u)$ $\}$\\
$\sem{\monoid,h,I}^{++}_p(u)$&= $\sup\{n+1~:~$there exists an $n$-over-computation of value in~$I$\\
		&\qquad\qquad of height at most~$p$ for~$\tilde h(u)$ $\}$
\end{tabular}
\end{center}
These four functions (for each $p$) are candidates to be recognised by $\monoid,h,I$.
The following lemma shows that if $p$ is sufficiently large, all the four functions
belong to the same cost function.
\begin{lemma}
For all~$p\geq 3|M|$, 
\begin{align*}
\sem{\monoid,h,I}^{--}_p\leq \sem{\monoid,h,I}^{-}_p\leq\sem{\monoid,h,I}^{+}_p\leq\sem{\monoid,h,I}^{++}_p\ .
\end{align*}
For all~$p$, there exists a polynomial~$\alpha$ such that
\begin{align*}
	\sem{\monoid,h,I}^{++}_p\leq\alpha\circ\sem{\monoid,h,I}^{--}_p\ .
\end{align*}
For all~$p\leq r$,
\begin{align*}
\sem{\monoid,h,I}^{--}_r&\leq\sem{\monoid,h,I}^{--}_p\ ,&\text{and}\quad\sem{\monoid,h,I}^{++}_p&\leq\sem{\monoid,h,I}^{++}_r\ .
\end{align*}
\end{lemma}
\begin{proof}
All the inequalities are direct consequences of the results of the previous section.

The middle inequality in the first equation simply comes from 
the fact that, thanks to Theorem~\ref{theorem:exists-computation},
the union of the set of integers over which range the infimum in the definition of $\sem{\monoid,h,I}^{+}_p$
with the set of integers over which range the supremum in the definition of $\sem{\monoid,h,I}^{-}_p$ 
is $\nats$. This suffices for justifying the middle inequality.
The first and last inequalities of the equation simply come from the fact
that each $n$-computation is in particular
an $n$-under-computation and an $n$-over-computation respectively.

The second line is directly deduced from Theorem~\ref{theorem:unicity-computations}.

The third statement  simply comes from the the fact that each $n$-under-computation
of height at most $p$ is also an $n$-under-computation of height $r$ (left inequality).
The same goes for over-computations.
\end{proof}
The main consequence of this lemma takes the form of a definition.
\begin{definition}\label{definition:recognisable}
For all stabilisation monoids $\monoid$, all mappings from an alphabet $\alphabet$
to~$M$, and all ideals $I$, there exists a unique cost function $\sem{\monoid,h,I}$
from $\alphabet^*$ to $\NI$ such that for all $p\geq 3|M|$, all the functions 
$\sem{\monoid,h,I}^{--}_p$,
$\sem{\monoid,h,I}^{-}_p$,
$\sem{\monoid,h,I}^{+}_p$ and
$\sem{\monoid,h,I}^{++}_p$ belong to $\sem{\monoid,h,I}$.
It is called the \intro{cost function recognised by $\monoid,h,I$}.
One sometimes also writes that it  is recognised by $\monoid$.
\end{definition}

\begin{example}\label{example:recognisable-size}
The cost function $|\cdot|_a$ is recognised 
by~$\monoid,\{a\mapsto a,b\mapsto b\},\set{0}$,
where $\monoid$ is the stabilisation monoid of Example~\ref{example:stabilisation-monoid-counta}.
In particular, the informal reasoning developed in the example such as ``a few+a few=a few''
now has a formal meaning: the imprecision in such arguments is absorbed in the
equivalence up to $\alpha$ of computation trees, and results in the fact that the monoid
does not define a unique function, but instead directly a cost function.
\end{example}

Another example is the case of standard regular languages.
\begin{example}\label{example:language-recognisable}
Let us recall that a monoid $\monoid$ together with $h$ from $\alphabet$ to $M$
and a subset $F\subseteq M$ is said to \intro{recognise} a language $L$ over $\alphabet$
if for all words $u$, $u\in L$ if and only if $\pi(\tilde h(u))\in F$.
The same monoid can be seen, thanks to Remark~\ref{remark:standard-monoid}
as a stabilisation monoid. In this case, thanks to Remark~\ref{remark:computations-standard},
the same $\monoid,h,F$ recognises the characteristic mapping of $L$.
\end{example}

An elementary result is also the closure under composition with a morphism.
\begin{myfact}\label{fact:recognisable-composition-morphism}
Let $\monoid,h,I$ recognise a cost function $f$ over $\alphabet^*$,
and let $z$ be a mapping from another alphabet $\alphabetB$ to $\alphabet$, then $\monoid,h\circ z,I$
recognises $f\circ \tilde z$.
\end{myfact}
\begin{proof}
One easily checks that the computations involved in the definition of $\sem{\monoid,h,I}^+(\tilde z(u))$
are exactly the same as the one involved in the definition of  $\sem{\monoid,h\circ z,I}^+(u)$.
\end{proof}

We continue this section by developing other tools for analysing the recognisable cost functions.

\subsection{The $\sharp$-expressions}
\label{subsection:sharp-expression}

We now present the notion of $\sharp$-expressions. This provides a convenient notation
in several situations. This object was introduced by
Hashiguchi for studying distance automata \cite{Hashiguchi82b}.
The $\sharp$-expressions can be seen in two different ways.
On one side, a $\sharp$-expression allows to denote an element in a stabilisation monoid.
On the other side, a $\sharp$-expression denotes an infinite sequence of words.
Such sequences are used as witnesses, {\it e.g.}, of the non-existence of a bound
for a function (if the function tends toward infinity over this sequence),
or of the non-divergence of a function $f$ (if the function is bounded over the sequence).
More generally, $\sharp$-expressions will be used as witnesses 
of non-domination.

In a finite monoid~$\monoid$, given an element $a\in M$,
one denotes by~$a^\omega$ the only idempotent which is a power of $a$.
This element does not exist in general for infinite monoids, while it always does
for finite monoids (our case). Furthermore, when it exists, it is unique.
In particular in a finite monoid $\monoid$, $a^\omega=a^\Omega$, where
$\Omega$ is some multiple of ${|M|!}$.
This is a useful notion since the operator of stabilisation is only defined
for idempotents. In a stabilisation monoid, let us denote by
$a^\osharp$ the element $(a^\Omega)^\sharp$.
As opposed to $a^\sharp$ which is not defined if $a$ is not idempotent,
$a^\osharp$ is always defined. We consider $\Omega$ as fixed from now.

A \intro{$\sharp$-expression} over a set~$A$ is
an expression composed of letters from $A$, products, and exponents with $\osharp$.
A $\sharp$-expression~$E$ over a stabilisation monoid denotes a computation
in this stabilisation monoid. It naturally evaluates to an element of $E$,
denoted~$\val(E)$, and called the \intro{value of $E$}.
A $\sharp$-expression is called \intro{strict} if it contains at least
one occurrence of~$\osharp$.

Given a set $A\subseteq M$, call \intro{$\langle A\rangle^\sharp$}
the set of values of expressions over~$A$.
Equivalently, it is the least set which contains $A$ and is closed under product and
stabilisation of idempotents. One also denotes
\intro{$\langle A\rangle^{\sharp{+}}$} the set of values of strict $\sharp$-expressions
over~$A$.

The~\intro{$n$-unfolding} of a $\sharp$-expression over~$A$ is
a word in~$A^+$ defined inductively as follows:
\begin{align*}
\unf(a,n)	&= a\\
\unf(EF,n)	&= \unf(E,n)\unf(F,n)\\
\unf(E^\osharp,n)	&=\overbrace{\unf(E,n)\dots\unf(E,n)}^{n~\text{times}}
\end{align*}

We conclude this section by showing how
$\sharp$-expressions can be used as witnesses of the behaviour
of a regular cost function.
\begin{proposition}\label{proposition:sharp-witness}
Assume~$\monoid,h,I$ recognises $f$, and
let~$E$ be a $\sharp$-expression over~$\alphabet$ of value~$a$, then:
\begin{itemize}
\item if~$a\in I$ then $\{f(\unf(E,\Omega n))~:~n\geq 1\}$ tends toward infinity,
\item if~$a\not\in I$ then $\{f(\unf(E,\Omega n))~:~n\geq 1\}$ is bounded.
\end{itemize}
\end{proposition}
\begin{proof}
We need, given a positive integer $n$, to produce an $n$-computation of value $a$.
It is defined as follows:
\begin{align*}
\computation(a,n)	  &= a\\
\computation(EF,n) &= \val(EF)[\computation(E,n),\computation(F,n)]\\
\computation(E^\osharp,n)&= \val(E^\osharp)[\overbrace{\computation(E^\Omega,n),\dots,\computation(E^\Omega,n)}^{n~\text{times}}]\\
\computation(E^1,n)&= \computation(E,n)\\
\computation(E^k,n)&= \val(E^k)[\computation(E,n),\computation(E^{k-1},n)]\tag{for $k>1$}
\end{align*}
It is easy to check that $\computation(E,n)$ is an~$n$-computation for~$\unf(u,\Omega n)$, that
its value is $\val(E)$ and that its height $H$ depends only upon $E$.
What we have is in fact stronger:
$\computation(E,n)$ is an $m$-computation for~$\unf(E,\Omega n)$ for all~$m\leq n$.

\begin{asparaitem}
\item
Let us suppose~$a\in I$.
We have:
\begin{align*}
\sem{\monoid,h,I}^{+}_{H}&=\sup\{m+1~:~\text{there is an $m$-computation for~$\tilde h(\unf(E,\Omega n))$ of value in~$I$}\}\\
	&\geq n\ .\tag{\text{using~$\computation(E,n)$ as a witness}}
\end{align*}
Thus~$f(\unf(E,\Omega n))$ tends toward infinity when $n$ tends to infinity.

\item 
Suppose now that if~$a\not\in  I$, one obtains:
\begin{align*}
\sem{\monoid,h,I}^{-}_{H}&=\inf\{m~:~\text{there is an $m$-computation
		for~$\tilde h(\unf(E,\Omega n))$ of value in~$M\setminus I$}\}\\
	&=0\ .\tag{\text{using~$\computation(E,n)$ as a witness}}
\end{align*}
Thus $\{f(\unf(E,n))~:~n\in\nats\}$ is bounded.
\end{asparaitem}
\end{proof}




\subsection{Quotients, sub-stabilisation monoids and products}
\label{subsection:morphisms}

We introduce here some useful definitions for manipulating and composing stabilisation
monoids. We use them for proving the closure of recognisable cost functions under
min and max (Corollary~\ref{corollary:rec-min-max}).

Let $\monoid=\langle M,\cdot,\sharp,\leq\rangle$
and $\monoid'=\langle M',\cdot',\sharp',\leq'\rangle$ be stabilisation monoids.
A \intro{morphism of stabilisation monoids}
from  $\monoid$ to $\monoid'$
is a mapping~$\mu$ from~$M$ to~$M'$ such that
\begin{itemize}
\item $\mu(1_\monoid)=1_{\monoid'}$,
\item $ \mu(x)\cdot' \mu(y) = \mu(x\cdot y)$ for all~$x,y$ in~$M$,
\item for all~$x,y$ in~$M$, if $x\leq y$ then $\mu(x)\leq' \mu(y)$,
\item $\mu(e)^{\sharp'} = \mu(e^\sharp)$ for all~$e\in E(\monoid)$
  (in this case, $\mu(e)\in E(\monoid')$).
\end{itemize}


\begin{remark}\label{remark:morphism}
The $n$-computations ({\it resp.}, $n$-under-computations, $n$-over-computations)
over~$\monoid$ are transformed by morphism (applied to each node of the tree)
into $n$-computations ({\it resp.}, $n$-under-computations, $n$-over-computations)
over~$\monoid'$.
In  a similar way, the image under morphism of a $\sharp$-expression
over~$\monoid$ is a~$\sharp$-expression over~$\monoid'$.
\end{remark}
We immediately obtain:
\begin{lemma}\label{lemma:morphism}
For $\mu$ a morphism of stabilisation monoids from
$\monoid$ to~$\monoid'$, $h$ a mapping 
from an alphabet~$\alphabet$ to~$\monoid$ and~$I'$ an ideal
of $\monoid'$, we have:
\begin{align*}
\sem{\monoid,h,\mu^{-1}(I')}&=\sem{\monoid',\mu\circ h,I'}\ .
\end{align*}
\end{lemma}
\begin{proof} Let us remark first that~$I=\mu^{-1}(I')$
is an ideal of~$\monoid$.

Let~$u$ be a word in~$\alphabet^*$.
Let us consider an $n$-computation over~$\monoid$ for~$\tilde h(u)$
of value~$a\in \mu^{-1}(I')$. This computation can be transformed
by morphism into an $n$-computation over~$\monoid'$
for $(\mu\circ h)(u)$  of value~$\mu(a)\in I'$.
In a similar way, each $n$-computation over~$\tilde h(u)$
of value~$a\in M\setminus \mu^{-1}(I')$
can be transformed into an $n$-computation of value
$\mu(a)\in M'\setminus I'$.
\end{proof}

The notion of morphism is intimately related to the notion of product.
Given two stabilisation monoids $\monoid=\langle M,\cdot,\sharp,\leq\rangle$
and~$\monoid'=\langle M',\cdot',\sharp',\leq'\rangle$,
one defines their \intro{product} by:
\begin{align*}
\monoid\times \monoid'&=\langle M\times M',\cdot'',\sharp'',\leq ''\rangle
\end{align*}
where $(x,x')\cdot''(y,y')=(x\cdot y,x'\cdot' y')$, $(e,e')^{\sharp''}=(e^\sharp,{e'}^{\sharp'})$,
and~$(x,x')\leq''(y,y')$ if and only if $x\leq y$ and~$x'\leq' y'$.

As expected, the projection over the first component
({\it resp.}, second component) is a morphism  of stabilisation monoids
from $\monoid\times\monoid'$ onto $\monoid$ ({\it resp.}, onto~$\monoid'$).
It follows by Lemma~\ref{lemma:morphism}
that if $f$ is recognised by~$\monoid,h,I$ and~$g$ by
$\monoid',h',I'$, then $f$ is also recognised
by~$\monoid\times\monoid',h\times h',I\times M'$
and $g$ by~$\monoid\times\monoid',h\times h',M\times I'$, 
in which one sets 
$(h\times h')(a) = (h(a),h(a'))$ for all letters~$a$.
Thus one obtains:
\begin{lemma}\label{lemma:joint-recognition}
If~$f$ and~$g$ are recognisable cost functions
over $\alphabet^*$,
there exist a stabilisation monoid~$\monoid$,
an application $h$ from~$\alphabet$ to~$\monoid$
and two ideals~$I,J$ such that~$\monoid,h,I$ recognises~$f$
and $\monoid,h,J$ recognises~$g$.
\end{lemma}
\begin{corollary}\label{corollary:rec-min-max}
If~$f$ and~$g$ are recognisable, then so are $\max(f,g)$
and $\min(f,g)$.
\end{corollary}
\begin{proof}
According to Lemma~\ref{lemma:joint-recognition},
one assumes $f$ recognised by $\monoid,h,I$ and~$g$ by~$\monoid,h,J$.
Then (for a height fixed to at most $p=3|M|$) one has:
\begin{align*}
\max&(\sem{\monoid,h,I}^{+}_p,\sem{\monoid,h,J}^{+}_p)(u)\\
&=\max\begin{cases}
	\sup\{n+1~:~\text{there is an $n$-computation for~$\tilde h(u)$ of value in~$I$}\}&\\
	\sup\{n+1~:~\text{there is an $n$-computation for~$\tilde h(u)$ of value in~$J$}\}
	\end{cases}\\
&=\sup\{n+1~:~\text{there exists an $n$-computation over~$\tilde h(u)$ of value in~$I\cup J$}\}\\
&=\sem{\monoid,h,I\cup J}^{+}_p\ .
\end{align*}
Thus  $\max(f,g)$ is recognised by~$\monoid,h,I\cup J$.
In a similar way, $\min(f,g)$ is recognised by~$\monoid,h,I\cap J$.
\end{proof}




\subsection{Decidability of the domination relation}
\label{subsection:domination-recognizable}

We are now ready to establish the
decidability of the domination relation.
\begin{theorem}\label{theorem:rec-domination}
The domination relation ($\preccurlyeq$) is decidable over
recognisable cost functions.
\end{theorem}
\begin{proof}
Let $f,g$ be recognisable cost functions.
According to Lemma~\ref{lemma:joint-recognition} 
there exist a stabilisation monoid~$\monoid$, a mapping~$h$
from the alphabet~$\alphabet$ to~$M$
and two ideals~$I,J$ such that~$\monoid,h,I$ recognises~$f$ and~$\monoid,h,J$
recognises~$g$.

We show that $f$ dominates $g$ if and only if the following (decidable) property holds:
\begin{align*}
\langle h(\alphabet)\rangle^\sharp\cap I\subseteq J\ .
\end{align*}

\noindent
{\em First direction.} Let us suppose
$\langle h(\alphabet)\rangle^\sharp\cap I\subseteq J$.
Of course, every $n$-computation over $\tilde h(u)$ for a word~$u$ over $h(\alphabet)$
has its value in $\langle h(\alphabet)\rangle^\sharp$.
It follows that (for heights at most $3|M|$):
\begin{align*}
\sem{\monoid,h,I}^{+}(u)&= \sup\{n+1~:~\text{there is an~$n$-computation for~$h(u)$ of value in~$I$}\}\\
 &\leq \sup\{n+1~:~\text{there is an~$n$-computation for~$h(u)$ of value in~$J$}\}\\
 &=\sem{\monoid,h,J}^{+}(u)\ .
\end{align*}
Thus we have $f\preccurlyeq g$.
\smallskip

\noindent
{\em Second direction.} Let us suppose the existence of
$a\in \langle h(\alphabet)\rangle^\sharp\cap I\setminus J$.
By definition of~$\langle h(\alphabet)\rangle^\sharp$,
there is a $\sharp$-expression $E$ over~$h(\alphabet)$ of value~$a$.
Let~$F$ be the $\sharp$-expression over~$\alphabet$ obtained by
substituting to each element~$x\in h(\alphabet)$ some
letter from~$c\in\alphabet$ such that~$h(c)=x$.
According to Proposition~\ref{proposition:sharp-witness}, $f$ is 
unbounded over~$\{\unf(F,\Omega n)~:~n\geq 1\}$ (for some suitable $k$).
However, still applying Proposition~\ref{proposition:sharp-witness},
$g$ is bounded over~$\{\unf(F,\Omega n)~:~n\geq 3\}$.
This witnesses that $g$ does not dominate~$f$.
\end{proof}


\subsection{Closure under $\inf$-projection}
\label{subsection:closure-inf-projection}

We establish the following theorem.
\begin{theorem}\label{theorem:inf-projection}
Recognisable cost functions are effectively closed under inf-projection.
\end{theorem}
The projection in the classical case (of recognisable languages of finite words) requires
a powerset construction (for monoids as for deterministic automata).
In our case, the approach is similar.
Let $z$ be a mapping from alphabet $\alphabet$ to $\alphabetB$.
The goal of a stabilisation monoid which would recognise the inf-projection by $z$ 
of a recognisable cost function is to keep track of all the values a computation
could have taken for some inverse image by $\tilde z$ of the input word.
Hence an element of the stabilisation monoid for the inf-projection of the
cost function consists naturally of a set of elements in the original monoid.

A closer inspection reveals that it is possible to close these subsets downward,
{\it i.e.}, to consider only ideals. In fact, it is not only possible, but it is even necessary
for the construction to go through. Let us describe more formally this construction.

We have to consider a construction of ideals.
Let~$M_\ideal$ be the set of ideals of $\monoid$.
One equips~$M_\ideal$ of an order simply by inclusion:
$$
I\leq J\qquad\text{if}\qquad I\subseteq J\ ,
$$
and of a product as follows:
\begin{align*}
A\cdot B\quad&=\quad\{a\cdot b~:~a\in A,~b\in B\}\ideal\ .
\end{align*}
Finally, the stabilisation is defined for an idempotent by:
\begin{align*}
E^\sharp&=\langle E \rangle^{\sharp+}\ideal\ .
\end{align*}
The resulting structure $\langle M_\ideal,\cdot,\leq,\sharp\rangle$
is denoted $\monoid_\ideal$.

It may seem a priori that our first goal would be to prove that
the structure defined in the above way is indeed a stabilisation monoid.
In fact, thanks to Proposition~\ref{proposition:unicity-to-axioms}, this
will be for free (see Lemma~\ref{lemma:ideal-is-stabilisation-monoids} below).

We now prove that $\monoid_\ideal$
can be used for recognising the inf-projection of a cost
function recognised by $\monoid$. Thus our goal is to relate
the (under)-computations in $\monoid_\ideal$ to the (under)-computations
in $\monoid$. This will provide a semantic link between the two stabilisation monoids.
This relationship takes the form of Lemmas~\ref{lemma:inf-key1}
and~\ref{lemma:inf-key2} below.

Let us first state a simple remark on the structure of idempotents.
\begin{lemma}\label{lemma:inf-idempotent}
If~$E$ is an idempotent in $M_\downarrow$, then for all~$a\in E$
there exist $b,c,e\in E$ with $e$ idempotent such that~$a\leq b\cdot e\cdot c$.
\end{lemma}
\begin{proof}
As~$E=\overbrace{E\cdots E}^{n~\text{times}}$, for all~$n\geq 1$, there exist~$a_1,\dots,a_n\in E$
such that $a\leq a_1\cdots a_n$.
Hence using Ramsey's theorem, for~$n$ sufficiently
large, there exist~$1<i\leq j< n$ such that~$a_i\cdots a_{j}=e$ is an idempotent.
One sets $b=a_1\cdots a_{i-1}$, $c=a_{j+1}\cdots a_n$. We have $b,c,e\in E$,
and $a\leq b\cdot e\cdot c$.
\end{proof}
A similar characterisation holds for the stabilisation of idempotents.
\begin{lemma}\label{lemma:inf-idempotent-stable}
If~$E$ is a stable idempotent in $M_\downarrow$ ({\it i.e.} such that $E=E^\sharp$), then for all~$a\in E$
there exist $b,c,e\in E$ with $e$ idempotent such that~$a\leq b\cdot e^\sharp\cdot c$.
\end{lemma}
\begin{proof}
By definition of $E^\sharp$, there is a strict $\sharp$-expression $F$ over $E$ such that $a\leq \val(F)$.
Thus it is sufficient to prove, by induction, that all strict $\sharp$-expressions $F$
is such that $\val(F)\leq b\cdot e^\osharp\cdot c$ for some $b,e,c$ in $E$.
The base case is $F=G^\osharp$ where $G$ is a non strict $\sharp$-expression.
In this case $\val(G)=g\in E$.
It follows that $\val(G^\osharp)=\val(G)^\osharp\leq g^\omega\cdot g^\osharp\cdot g^\omega$.
Thus the induction hypothesis holds. The other case is the product $F=GH$.
By induction hypothesis, $\val(G)\leq a\cdot e^\osharp\cdot b$ and
$\val(H)\leq a'\cdot f^\osharp\cdot b'$. It follows that  $\val(F)\leq a\cdot e^\osharp\cdot d$
with $d=a'\cdot f ^\osharp\cdot b'\in E$. Once more the induction hypothesis hold.
\end{proof}

\begin{lemma}\label{lemma:inf-key1}
Let~$A_1\dots A_k$ be a word over~$M_\ideal$ and let $T$ be an $n$-under-computation
over $A_1\dots A_k$ of height at most~$p$ and of value~$A$.
For all~$a\in A$, there exists an $n$-under-computation of height~$3p$ and value~$a$
for some word~$a_1\dots a_k$ such that $a_1\in A_1$,\dots,$a_k\in A_k$.
\end{lemma}
\begin{proof}
The proof is by induction on~$p$.
\medskip

\noindent
\emph{Leaf case}, {\it i.e.}, $T=A_1$. Let~$a\in A\subseteq A_1$, then $a$ is an $n$-computation of value~$a\in A$.
\medskip


\noindent
\emph{Binary node}, {\it i.e.},  $T=A[T_1,T_2]$. Let $B_1$ and $B_2$
be the respective values of $T_1$ and $T_2$.
Let~$a\in A\subseteq B_1\cdot B_2$. By definition of the product, there exists~$b_1\in B_1$
and~$b_2\in B_2$ such that~$a\leq b_1\cdot b_2$.
By induction hypothesis, there exist $n$-under-computations~$t_1$ and~$t_2$
of respective values~$b_1$ and~$b_2$.
The $n$-under-computation $a[t_1,t_2]$ satisfies the induction hypothesis.
\medskip


\noindent
\emph{Idempotent node.}
$T=F[T_1,\dots,T_k]$ for some~$k\leq n$ where $F\subseteq E$
	for an idempotent $E$ such that the value of $T_i$ is $E$ for all~$i$.
	Let~$a\in F\subseteq E$.
	We have $a\leq b\cdot e\cdot c$ for some $b,c,e\in E$ (Lemma~\ref{lemma:inf-idempotent}).
	We then apply the induction hypothesis for~$b,e,\dots,e$ and~$c$
	on the $n$-under-computations~$T_1,\dots,T_{k-1}$ and $T_k$ respectively,
	yielding the $n$-under-computations $t_1,\dots,t_{k-1}$ and $t_k$ respectively.
	The tree $a[t_1,(e\cdot c)[e[t_2,\dots,t_{k-1}],t_k]]$ is an $n$-under-computation
	witnessing that the induction hypothesis holds.
\medskip

\noindent
\emph{Stabilisation node.}
$T=F[T_1,\dots,T_k]$ for some~$k> n$ and $F\subseteq E^\sharp$ for some idempotent $E$
	such that the value of $T_i$ is $E$ for all~$i$.
	Let~$a\in F\subseteq E^\sharp$.
	We have $a\leq b\cdot e^\sharp\cdot c$ for some $b,e,c\in E$ (Lemma~\ref{lemma:inf-idempotent-stable}).
	We then apply the induction hypothesis for~$b,e,\dots,e$ and~$c$ respectively
	and the computations~$T_1,\dots,T_k$ respectively,
	yielding the $n$-under-computations $t_1,\dots,t_k$ respectively.
	We conclude by constructing the 
	$n$-under-computation~$a[t_1,(e^\sharp\cdot c)[e^\sharp[t_2,\dots,t_{k-1}],t_k]]$
	(remark that $e^\sharp[t_2,\dots,t_{k-1}]$ is a valid under-computations since
	$e^\sharp\leq e$).
\end{proof}



\begin{lemma}\label{lemma:inf-key2}
There exists a polynomial $\alpha$ such that 
for all words~$A_1\dots A_k$ over~$M_\ideal$ and all $\alpha(n)$-over-computation $T$ 
for~$A_1\dots A_k$ of height~$p$ and value~$A$,
and all $a_1\in A_1,\dots,a_k\in A_k$,
there exists an~$n$-computation over~$a_1\dots a_k$ of value~$a\in A$ and of height at most~$3|M|p$.
\end{lemma}
\begin{proof}
The proof is by induction on $p$. Set $\alpha(n)=n^{3|M|}$ for all $n$.
\medskip

\noindent
\emph{Leaf case,} {\it i.e.}, $T=A$ and~$u=a_1\in A_1\subseteq A$. Hence~$a_1$ is a computation
satisfying the induction hypothesis.
\medskip

\noindent
\emph{Binary node,} {\it i.e.}, $T=A[T_1,T_2]$ where $T_1$ and $T_2$ have respective
	values $B_1$ and $B_2$ such that $B_1\cdot B_2\subseteq A$. One applies the induction
	hypothesis on $T_1$ and $T_2$, and gets computations $t_1$
	and $t_2$, of respective values $b_1\in B_1$ and $b_2\in B_2$.
	The induction hypothesis is then fulfilled with the $n$-computation
	 $(b_1\cdot b_2)[t_1,t_2]$ of value~$b_1\cdot b_2\in A$.
\medskip

\noindent
\emph{Idempotent node,} {\it i.e.},
	$T=F[T_1,\dots,T_k]$ for~$k\leq n^{3|M|}$ where $T_1,\dots,T_k$
	share the same idempotent value $E\subseteq F$.
	Let~$t_1,\dots,t_k$ be the $n$-computations of respective values $b_1,\dots,b_k$
	obtained by applying the induction hypothesis
	on $T_1,\dots,T_k$ respectively. Furthermore, according to Theorem~\ref{theorem:exists-computation},
	there exists an $n$-computation $t$ for the word $b_1\dots b_k$ of height at most $3|M|$.
	Let $a$ be the value of $t$. Since $E$ is an idempotent, it is closed under product and stabilisation
	and contains $b_1,\dots,b_k$. It follows that $a\in E$ (by induction on the height of $t$).
	The induction hypothesis holds using the witness $n$-computation $t\{t_1,\dots,t_k\}$
	where $t\{t_1,\dots,t_k\}$ is obtained from $t$ by substituting the $i$th leaf for $t_i$ for all~$i=1\dots k$.
\medskip

\noindent
\emph{Stabilisation node,} {\it i.e.},
	$T=F[T_1,\dots,T_k]$ for~$k> n^{3|M|}$ where $T_1,\dots,T_k$
	all share the same idempotent value $E$ such that $E^\sharp\subseteq F$.
	Let~$t_1,\dots,t_k$ be the $n$-computations of respective values $b_1,\dots,b_k$ obtained by applying
	the induction hypothesis on $T_1,\dots,T_k$ respectively.
	Furthermore, according to Theorem~\ref{theorem:exists-computation},
	there exists an $n$-computation $t$ for $b_1\dots b_k$ of height at most $3|M|$.
	Since $t$ has height at most $3|M|$ and has more than $n^{3|M|}$ leaves,
	it contains at least one node of degree more than $n$, namely, a  stabilisation node.
	It is then easy to prove by induction on the height of $t$ that the value of $t$
	belongs to $\langle E\rangle^{\sharp+}$.
	Thus the $n$-computation $t\{t_1,\dots,t_k\}$ (as defined in the above case) is a witness
	for the induction hypothesis.
\end{proof}

\begin{lemma}\label{lemma:ideal-is-stabilisation-monoids}
$\monoid_\ideal$ is a stabilisation monoid.
\end{lemma}
\begin{proof}
Consider an $n$-under-computation $T$ of value $A$ in $\monoid_\ideal$
for some word $A_1\dots A_k$ of height at most $p$,
and some $\alpha(n)$-over-computation $T'$ for the
same word of value $B$ (with $\alpha(n)=\alpha'(n)^{3|M|}$ where $\alpha'$
	is obtained from Theorem~\ref{theorem:unicity-computations} applied to $\monoid$ for height at most $3p$).
We aim at $A\leq B$. Indeed, this implies that one can use Proposition~\ref{proposition:unicity-to-axioms},
and get that $\monoid_\ideal$ is a stabilisation semigroup (it is then straightforward to
prove it a stabilisation monoid. 

Let $a\in A$, we aim at $a\in B$, thus proving $A\subseteq B$, {\it i.e.}, $A\leq B$.
By Lemma~\ref{lemma:inf-key1}, there exists
an $n$-under-computation for some word $a_1\dots a_k$ with $a_1\in A_1,\dots,a_k\in A_k$,
of height at most $3p$ and value $a$.
Applying Lemma~\ref{lemma:inf-key2} on $T'$, there exists an $\alpha'(n)$-over-computation
for the same word $a_1\dots a_k$ of value $b\in B$. Then applying Theorem~\ref{theorem:unicity-computations},
we get $a\leq b$. Hence $a\in B$ since $B$ is downward closed.
\end{proof}

We can now establish the result of this section.
\begin{proof}[Proof of Theorem~\ref{theorem:inf-projection}]
Assume a function $f$ over the alphabet $\alphabet$
is recognised by~$\monoid,h,I$,
and let~$z$ be some mapping from~$\alphabet$ to~$\alphabetB$.
Let $H$ be the mapping from $\alphabetB$ to $M_\ideal$ 
which to $b\in\alphabetB$ associates $h(z^{-1}(b))\ideal$,
and let~$K\subseteq M_\ideal$ be
$$
K=\{J\in M_\ideal~:~J\subseteq I\}\ .
$$
We shall prove that $M_\ideal,H,K$ recognise the cost function of $f_{\inf,z}$.
There are two directions.

Consider a word $u=b_1\dots b_k$ over alphabet $\alphabetB$ such that
$$\sem{\monoid_\ideal,H,K}^{--}_{3|M_\ideal|}(u)\leq n\ .$$
This means that there exists an $\alpha(n)$-under-computation over $A_1\dots A_k=\tilde H(u)$
of value $J\in M_\ideal\setminus K$, and height at most $3|M_\ideal|$. 
By definition of $K$, this means that there exists some $a\in J\setminus I$.
Let us apply now Lemma~\ref{lemma:inf-key1}, and obtain
an $n$-under-computation for some $a_1\dots a_k$ of value $a\in A$,
and of height at most $d=9|M_\ideal|$, where $a_i\in A_i$ for all $i=1\dots k$.
By definition of $H$, there exists $c_i\in\alphabet$ such that $z(c_i)=b_i$ and $h(c_i)=a_i$.
Thus, set $v=c_1\dots c_k$. The word $v$ is such that $\tilde z(v)=u$ and $\sem{\monoid,h,I}_d^{--}(v)\leq n$.
This a witness that 
$$
(\sem{\monoid,h,I}_d^{--})_{\inf,z}(u)\leq n\ .
$$

Conversely, consider a word $u$ over the alphabet $\alphabetB$
such that
$$\sem{\monoid_\ideal,H,K}^{++}_{3|M_\ideal|}(u)\geq \alpha(n)+1\ ,$$
where $\alpha$ is the polynomial obtained from Lemma~\ref{lemma:inf-key2}.
This means that there exists an $\alpha(n)$-over-computation for the word $A_1\dots A_k=\tilde H(u)$ of height
at most $3|M_\ideal|$ and value $J\in K$. 
Consider now some word $v=c_1\dots c_k$ over the alphabet $\alphabet$
such that $\tilde z(v)=u$. Let $a_1\dots a_k=\tilde h(v)$.
according to Lemma~\ref{lemma:inf-key2} there exists an $n$-computation for $a_1\dots a_k$
of height at most $d=9|M||M_\ideal|$ and value $a\in J$. Since by definition of $K$, $J\subseteq I$,
this means that $a\in I$. 
Thus, this computation witnesses that $\sem{\monoid,h,I}^{+}_{d}(v)\geq n$.
Since this this holds for all words $v$ such that $\tilde z(v)=u$, we obtain that
$$
(\sem{\monoid,h,I}^{+}_{d})_{\inf,z}(u)\geq n\ .
$$
\end{proof}




















\subsection{Closure under $\sup$-projection}
\label{subsection:closure-sup-projection}
We now establish the closure under sup-projection, using a proof
very similar to the previous section.

\begin{theorem}\label{theorem:sup-projection}
Recognisable cost functions are effectively closed under sup-projection.
\end{theorem}

The closure under $\sup$-projection follows the same principle as the
closure under $\inf$-projection. It uses also a powerset construction.
However, since everything is reversed, this is a construction of co-ideals.
A \intro{co-ideal} is a subset of a stabilisation monoid which is upward closed.
Let~$\monoid_\coideal$ be set of co-ideals over a given stabilisation
monoid~$\monoid$.
Given a set $A$, let us denote by~$A\coideal$ 
the least co-ideal containing~$A$, {\it i.e.}, $A\coideal=\{y~:~y\geq x\in A\}$.
One equips~$\monoid_\coideal$ of an order by:
$$
I\leq J\qquad\text{if}\quad I\supseteq J\ ,
$$
of a product with:
\begin{align*}
A\cdot B\quad&=\quad\{a\cdot b~:~a\in A,~b\in B\}\coideal\ ,
\end{align*}
and of a stabilisation operation by:
\begin{align*}
E^\sharp&=\langle E \rangle^{\sharp+}\coideal\ .
\end{align*}
Let us call $\monoid_\coideal$ the resulting structure. You can remark that $\langle E \rangle^{\sharp+}\coideal=\langle E \rangle^{\sharp}\coideal$. This was not the case for ideals. 
The proof is extremely close to the case of $\inf$-projection.
However, a careful inspection would show that all computations of bounds, and even 
some local arguments need to be modified.

Let us state a simple remark on the structure of idempotents.
\begin{lemma}\label{lemma:sup-idempotent}
If~$E$ is an idempotent in $M_\uparrow$, then for all~$a\in E$
there exist $b,c,e\in E$ with $e$ idempotent
such that $a\geq b\cdot e\cdot c$.
\end{lemma}
\begin{proof} 
As~$E=E\cdots E$, for all~$n$, there exist~$a_1,\dots,a_n\in E$
such that $a\geq a_1\cdots a_n$. Using Ramsey's theorem, for~$n$ sufficiently
large, there exist~$1<i\leq j< n$ such that~$a_i\cdots a_{j}=e$ is an idempotent.
One sets $b=a_1\cdots a_{i-1}$, $c=a_{j+1}\cdots a_n$. We have $b,c,e\in E$,
and $a\geq b\cdot e\cdot c$.
\end{proof}

Our second preparatory lemma is used for the treatment of stabilisation nodes.
\begin{lemma}\label{lemma:sup-stabilisation}
There exists a polynomial $\alpha$
such that for all idempotents~$E$ of $M_\uparrow$, all~$a\in E^\sharp$
and all $\alpha(m)\leq n$, there exists
an $m$-over-computation of height at most $2|M|+3$ of value $a$ over some word over $E$
of length $n$.
\end{lemma}
\begin{proof} 
It is sufficient to prove the result for a single pair $E,a$, and construct for each such case
a polynomial $\alpha_{E,a}$. Then, since there are finitely many such pairs $(E,a)$, one can choose a polynomial $\alpha$
that is above all the $\alpha_{E,a}$. This $\alpha$ will witness the lemma for all choices of $E$ and $a$.

We first claim $(\star)$ that if $b\in E$ then for all $n\geq 1$, there exists a word $w_n$ over $E$ of length
$n$ such that for all $m\geq 1$ there exist an $m$-over-computation for $w$ of height at most~$3$ of value $b$.
Indeed, by Lemma~\ref{lemma:sup-idempotent},
$b\geq c\cdot f\cdot d$ where $c,f,d$ belong to $E$, and $f$ is idempotent.
So if $n=1$, we take $w=b$. If $n=2$, we take $w=c(f \cdot d)$.
Finally, for $n\geq 3$, there is a natural $m$-over-computation of value $c\cdot f\cdot d$ of height $2$ or $3$ over
the word $c\underbrace{f\dots f}_{n-2~\text{times}}d$, which is of length $n$.

Consider now a $\sharp$-expression $e$ of value $a\in E^\sharp$ for some idempotent $E$.
Without loss of generality, we can choose it of height at most $2|M|$.
and consider the word $u_m=\unf(e,|M|!(m+1))$ for all $m\geq 1$.
The length of this word is a polynomial $\alpha(m)$, and there is an $m$-over-computation of height at most $2|M|$
of value $a$ for this word.
Consider now some~$n\geq\alpha(m)$. The word $u_m$ can be written $vb$ for some $b\in E$. We can apply the above claim to 
$b$ and $n+1-\alpha(m)$, yielding the word $w_{n+1-\alpha(m)}$. Combining the two $m$-over-computations, we then naturally obtain an $m$-over-computation for the word $vw_{n+1-\alpha(m)}$ of height at most $2|M|+3$ and of value $a$, and this word has length $n$.
\end{proof}




\begin{lemma}\label{lemma:sup-key1}
There exists a polynomial $\alpha$ such that for all
words $A_1\dots A_k$ over~$\monoid_\coideal$ and all  $\alpha(n)$-over-computations $T$
for $A_1\dots A_k$ of height at most~$p$ of value~$A$
and all~$a\in A$, there exists an $n$-over computation of height at most $(2|M|+3)p$ and value~$a$
for some word~$a_1\dots a_k$ with $a_1\in A_1$,\dots,$a_k\in A_k$.
\end{lemma}
\begin{proof}
The proof is by induction on~$p$. We take the polynomial $\alpha$ of Lemma~\ref{lemma:sup-stabilisation}.
\medskip

\noindent
\emph{Leaf case}, {\it i.e.}, $T=A_1$. Let~$a\in A\subseteq A_1$, then $a$ is an $n$-computation of value~$a\in A$.
\medskip


\noindent
\emph{Binary node}, {\it i.e.},  $T=A[T_1,T_2]$. Let $B_1$ and $B_2$
be the respective values of $T_1$ and $T_2$.
Let~$a\in A\subseteq B_1\cdot B_2$. By definition of the product, there exists~$b_1\in B_1$
and~$b_2\in B_2$ such that~$a\geq b_1\cdot b_2$.
By induction hypothesis, there exist $n$-computations~$t_1$ and~$t_2$
of respective values~$b_1$ and~$b_2$.
The $n$-over-computation $a[t_1,t_2]$ satisfies the induction hypothesis.
\medskip

\noindent
\emph{Idempotent node.}
$T=F[T_1,\dots,T_k]$ for some~$k\leq\alpha(n)$ where $F\subseteq E$
	for an idempotent $E$ such that the value of $T_i$ is $E$ for all~$i$.
	Let~$a\in F\subseteq E$.
	We have $a\geq b\cdot e\cdot c$ for some $b,c,e\in E$ (Lemma~\ref{lemma:sup-idempotent}).
	We then apply the induction hypothesis for~$b,e,\dots,e$ and~$c$
	on the computations~$T_1,\dots,T_{k-1}$ and $T_k$ respectively,
	yielding the $n$-under-computations $t_1,\dots,t_{k-1}$ and $t_k$ respectively.
	We conclude by constructing the 
	$n$-under-computation~$a[t_1,(e\cdot c)[e[t_2,\dots,t_{k-1}],t_k]]$.
\medskip

\noindent
\emph{Stabilisation node.}
$T=F[T_1,\dots,T_k]$ for some~$k>\alpha(n)$ and $F\subseteq E^\sharp$ for some idempotent $E$
	such that the value of $T_i$ is $E$ for all~$i$.
	Let~$a\in F\subseteq E^\sharp$.
	According to Lemma~\ref{lemma:sup-stabilisation}, there exists a word $a_1\dots a_k$ over $E$
	and an $n$-over-computation~$t$ for $a_1\dots a_k$ of value $a$ and height at most $2|M|+3$.
	We then apply the induction hypothesis for each of $a_1,\dots, a_k$ with the computations~$T_1,\dots,T_k$ respectively.
	This yields $n$-over-computations $t_1,\dots,t_k$ respectively.
	We conclude by constructing the 
	$n$-over-computation obtained by substituting in $t$ the $i$th leaf with $t_i$.
\end{proof}





\begin{lemma}\label{lemma:sup-key2}
Let~$A_1\dots A_k$ be a word over~$\monoid_\coideal$ and $T$ be an $n$-under-computation~$T$
for~$A_1\dots A_k$ of height~$p$ and value~$A$.
For all words~$u=a_1\dots a_k$ with  $a_1\in A_1,\dots,a_k\in A_k$,
there exists an~$n$-computation over~$a_1\dots a_k$ of value~$a\in A$ and of height at most~$3|M|p$.
\end{lemma}
\begin{proof}
The proof is by induction on $p$.
\medskip

\noindent
\emph{Leaf case,} {\it i.e.}, $T=A$ and~$u=a_1\in A_1\subseteq A$. Hence~$a_1$ is a computation
satisfying the induction hypothesis.
\medskip

\noindent
\emph{Binary node,} {\it i.e.}, $T=A[T_1,T_2]$ where $T_1$ and $T_2$ have respective
	values $B_1$ and $B_2$ such that $B_1\cdot B_2\subseteq A$. One applies the induction
	hypothesis on $T_1$ and $T_2$, and get computations $t_1$
	and $t_2$, of respective values $b_1\in B_1$ and $b_2\in B_2$.
	The induction hypothesis is then fulfilled with the $n$-computation
	 $(b_1\cdot b_2)[t_1,t_2]$ of value~$b_1\cdot b_2\in A$.
\medskip

\noindent
\emph{Idempotent node,} {\it i.e.},
	$T=F[T_1,\dots,T_k]$ for~$k\leq n$ where $T_1,\dots,T_k$
	share the same idempotent value $E\subseteq F$.
	Let~$t_1,\dots,t_k$ be the $n$-computations of respective values $b_1,\dots,b_k$
	obtained by applying the induction hypothesis
	on $T_1,\dots,T_k$ respectively. Furthermore, according to Theorem~\ref{theorem:exists-computation},
	there exists an $n$-computation $t$ for the word $b_1\dots b_k$ of height at most $3|M|$.
	Let $a$ be the value of $t$. Since $E$ is an idempotent, it is closed under product
	and contains $b_1,\dots,b_k$. Since furthermore $t$ does not contain any node of stabilisation,
	we obtain that $a\in E$ (by induction on the height of $t$).
	We conclude using the $n$-computation $t\{t_1,\dots,t_k\}$ (obtained from $t$ by substituting
	the $i$th leaf of $t$ for $t_i$) which satisfies the induction hypothesis.
\medskip

\noindent
\emph{Stabilisation node,} {\it i.e.},
	$T=F[T_1,\dots,T_k]$ for~$k> n$ where $T_1,\dots,T_k$
	all share the same idempotent value $E\subseteq F$.
	Let~$t_1,\dots,t_k$ be the $n$-computations of respective values $b_1,\dots,b_k$ obtained by applying
	the induction hypothesis on $T_1,\dots,T_k$ respectively.
	Furthermore, according to Theorem~\ref{theorem:exists-computation},
	there exists an $n$-computation $t$ for $b_1\dots b_k$ of height at most $3|M|$ and value $a$.
	Since $E^\sharp$ is a sub-stabilisation monoid of $\monoid$ which contains $b_1,\dots,b_k$,
	$a$ also belongs to $E^\sharp$.
	Thus the $n$-computation $t\{t_1,\dots,t_k\}$ satisfies the induction hypothesis.
\end{proof}


\begin{lemma}\label{lemma:coideal-is-stabilisation-monoids}
$\monoid_\coideal$ is a stabilisation monoid.
\end{lemma}
\begin{proof}
Consider an $n$-under-computation $T$ of value $A$ in $\monoid_\coideal$
for some word $A_1\dots A_k$ of height at most $p$,
and some $\alpha(n)$-over-computation $T'$ for the
same word of value $B$ (with $\alpha(n)=\alpha'(n)+2$ where $\alpha'$
	is obtained from Theorem~\ref{theorem:unicity-computations} applied to $\monoid$ for height at most $3p$).
We aim at $A\leq B$, which means $A\supseteq B$. Indeed, this implies that one can use Proposition~\ref{proposition:unicity-to-axioms},
and get that $\monoid_\coideal$ is a stabilisation monoid.

Let $b\in B$, we aim at $b\in A$, thus proving $B\subseteq A$, {\it i.e.}, $A\leq B$.
By Lemma~\ref{lemma:sup-key1}, there exists
an $\alpha'(n)$-over-computation for some word $a_1\dots a_k$ with $a_1\in A_1,\dots,a_k\in A_k$,
of height at most $3p$ and value $b$.
Applying Lemma~\ref{lemma:sup-key2} on $T$, there exists an $n$-computation
for the same word $a_1\dots a_k$ of value $a\in A$. Then applying Theorem~\ref{theorem:unicity-computations},
we get $a\leq b$. Hence $b\in A$ since $A$ is upward closed.
\end{proof}


We are ready to complete the proof of closure under sup-projection.
\begin{proof}{Proof of Theorem~\ref{theorem:sup-projection}}
Assume a function $f$ over the alphabet $\alphabet$
is recognised by~$\monoid,h,I$
and let~$z$ be some mapping from~$\alphabet$ to~$\alphabetB$.
Construct $H$ from $\alphabetB$ to $M_\coideal$ that maps
$b\in\alphabetB$ to $h(z^{-1}(b))\coideal$,
and let~$K\subseteq M_\coideal$ be
$$
K=\{J\in M_\coideal~:~J\cap I\neq \emptyset\}\ .
$$
Let us prove that $\monoid_\coideal,H,K$ recognises the cost function of $f_{\sup_z}$.

Consider now a word $u=b_1\dots b_k$ over $\alphabetB$.
Assume 
$$\sem{\monoid_\coideal,H,K}^{++}_{3|M_\coideal|}(u)\geq \alpha(n)+1\ ,$$
where $\alpha$ is the polynomial from Lemma~\ref{lemma:sup-key1}.
This means that there is an $\alpha(n)$-over-computation for~$H(b_1)\dots H(b_k)$ of value~$J\in K$
of height at most $3|M_\coideal|$.
By definition of $K$, there exists $a\in J\cap I$. Hence, by Lemma~\ref{lemma:sup-key1} ,
there exists an $n$-over-computation of height at most $d=(2|M|+3)2|M_\coideal|$ of value $a$
for some $a_1\dots a_k$ with $a_1\in H(b_1),\dots,a_k\in H(b_k)$.
By definition of $H$, this means that there exist $c_i\in\alphabet$ such that $a_i=h(c_i)$ and $z(c_i)=b_i$ for all $i=1\dots k$.
The obtained word $v=c_1\dots c_k$ is such that $\tilde z(v)=u$, and $\sem{\monoid,h,I}^{++}_{d}(v)\geq n$.
This witnesses that
$$
(\sem{\monoid,h,I}^{++}_{d})_{\sup,z}(u)\geq n\ .
$$

For the converse direction, consider a word $u=b_1\dots b_k$ over $\alphabetB$ such that 
$$\sem{\monoid_\coideal,H,K}_{3|M_\coideal|}^{--}(u)\leq n\ .$$
This means that there exists an $n$-under-computation for $A_1\dots A_k=\tilde H(b_1\dots b_k)$ of value $J\not\in K$,
and height at most $3|M_\coideal|$. 
Let $v=c_1\dots c_k$ be some word over $\alphabet$ such that $\tilde z(v)=u$.
By definition of $H$, this means that $a_i=h(c_i)\in H(b_i)$ for all $i=1\dots k$.
Thus, by Lemma~\ref{lemma:sup-key2}, there exists an $n$-computation for $a_1\dots a_k$
of value in $a\in J$ of height at most $d=9|M||M_\coideal|$.
Since $J\not\in K$, this means that $J\cap I=\emptyset$. As a consequence $a\in M\setminus I$.
It follows that $\sem{\monoid,h,I}^{-}_d(v)\leq n$. Since this holds for all $v$ such that $\tilde z(v)=u$, we get
$$(\sem{\monoid,h,I}^{-}_d)_{\sup,z}(u)\leq n\ .$$
\end{proof}








